Using Large Language Models to Generate JUnit Tests: An Empirical Study

A code generation model generates code by taking a prompt from a code comment, existing code, or a combination of both. Although code generation models (e.g., GitHub Copilot) are increasingly being adopted in practice, it is unclear whether they can successfully be used for unit test generation without fine-tuning for a strongly typed language like Java. To fill this gap, we investigated how well three models (Codex, GPT-3.5-Turbo, and StarCoder) can generate unit tests. We used two benchmarks (HumanEval and Evosuite SF110) to investigate the effect of context generation on the unit test generation process. We evaluated the models based on compilation rates, test correctness, test coverage, and test smells. We found that the Codex model achieved above 80% coverage for the HumanEval dataset, but no model had more than 2% coverage for the EvoSuite SF110 benchmark. The generated tests also suffered from test smells, such as Duplicated Asserts and Empty Tests.

==> Code/background_unit_test.tex <==
\begin{listing}[H]
{
\begin{PythonSourceCode*}{label=\textcolor{black}{\tiny{sum\_product.py}},highlightlines={14-16}}
def sum_product(numbers: List[int]) -> Tuple[int, int]:
    """ For a given list of integers, 
    return a tuple consisting of a sum and a product 
    of all the integers in a list.
    Empty sum should be equal to 0 and empty product 
    should be equal to 1.
    """
    sum_value = 0
    prod_value = 1
    for n in numbers:
        sum_value += n
        prod_value *= n
    return sum_value, prod_value
def test_0():
    result = sum_product([1, 2, 3, 4])
    assert result == (10, 24)
\end{PythonSourceCode*}
}
\caption{Unit Test Example}\label{lst:exampleunittest}
\end{listing}

==> Code/filter_integers.tex <==
% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/filter_integers.pdf}
%     \caption{Sample file from the HumanEval dataset~\cite{chen21}}
%     \label{fig:filter_integers}
% \end{figure}


\begin{listing}[H]
\centering
\includegraphics[width=\linewidth]{Figures/filter_integers.pdf}\vspace{-15pt}    
\caption{Sample file from the HumanEval dataset~\cite{chen2021codex}}
\label{lst:filter_integers}
\end{listing}

==> Code/generated_test_cases_java.tex <==
\begin{listing}[H]
{\renewcommand\theFancyVerbLine{%
\rmfamily\tiny\ifnum\value{FancyVerbLine}=25
  \setcounter{FancyVerbLine}{32}\ldots
\else
\arabic{FancyVerbLine}%
\fi
}
\begin{JavaSourceCode*}{label=\textcolor{black}{\tiny{TruncateNumber.java}},highlightlines={19-19}, firstnumber=19}
// Create 10 test cases for the above function
public List<Object[]> test_Cases = new ArrayList<>(){
    {
        add(new Object[]{3.5, 0.5});
        add(new Object[]{1.33, 0.33});
        add(new Object[]{123.456, 0.456});
        // remaining input-output examples hidden
    }
};
\end{JavaSourceCode*}
}
\caption{Using GitHub Copilot to generate framework-agnostic test cases (input/output pairs) for Java}\label{lst:generated_test_cases_java}
\end{listing}

==> Code/generated_test_cases_python.tex <==
\begin{listing}[H]
{\renewcommand\theFancyVerbLine{%
\rmfamily\tiny\ifnum\value{FancyVerbLine}=18 
  \setcounter{FancyVerbLine}{24}\ldots
\else
\arabic{FancyVerbLine}%
\fi
}
\begin{PythonSourceCode*}{label=\textcolor{black}{\tiny{filter\_integers.py}},highlightlines={13-13}, firstnumber=13}
# Create 10 test cases for the above function
test_cases = [
    (['a', 3.14, 5], [5]),
    ([1, 2, 3, 'abc', {}, []], [1, 2, 3]),
    ([1, 2, 3, 'abc', {}, [], 'def'], [1, 2, 3]),
    # remaining input-output examples hidden
]
\end{PythonSourceCode*}
}
\caption{Using GitHub Copilot to generate framework-agnostic test cases (input/output pairs) for Python}\label{lst:generated_test_cases}
\end{listing}

==> Code/generated_unit_tests.tex <==
\begin{listing}[H]
{\renewcommand\theFancyVerbLine{%
\rmfamily\tiny\ifnum\value{FancyVerbLine}=40 
  \setcounter{FancyVerbLine}{41}\ldots
\else
\arabic{FancyVerbLine}%
\fi
}
\begin{PythonSourceCode*}{label=\textcolor{black}{\tiny{filter\_integers.py}},highlightlines={27-27}, firstnumber=27}
# write pytest functions using the test_Cases array
def test_answer_0():
    result = filter_integers(test_cases[0][0])
    assert result == test_cases[0][1]

def test_answer_1():
    result = filter_integers(test_cases[1][0])
    assert result == test_cases[1][1]

def test_answer_2():
    result = filter_integers(test_cases[2][0])
    assert result == test_cases[2][1]
    
# remaining test functions are hidden
\end{PythonSourceCode*}
}
\caption{\footnotesize Using GitHub Copilot to generate \texttt{pytest} unit test}\label{lst:generated_unit_test_cases}
\end{listing}

==> Code/generated_unit_tests_java.tex <==
\begin{listing}[H]
{\renewcommand\theFancyVerbLine{%
\rmfamily\tiny\ifnum\value{FancyVerbLine}=51 
  \setcounter{FancyVerbLine}{52}\ldots
\else
\arabic{FancyVerbLine}%
\fi
}
\begin{JavaSourceCode*}{label=\textcolor{black}{\tiny{TruncateNumber.java}},highlightlines={34-34}, firstnumber=34}
    // write JUnit functions using the test_Cases array
    @Test
    public void test_0(){
        assertEquals(test_Cases.get(0)[1], 
        truncateNumber((Double) test_Cases.get(0)[0]));
    }
    @Test
    public void test_1(){
        assertEquals(test_Cases.get(1)[1], 
        truncateNumber((Double) test_Cases.get(1)[0]));
    }
    @Test
    public void test_2(){
        assertEquals(test_Cases.get(2)[1], 
        truncateNumber((Double) test_Cases.get(2)[0]));
    }
    
    // remaining test functions are hidden
\end{JavaSourceCode*}
}
\caption{\footnotesize Using GitHub Copilot to generate \texttt{JUnit} unit test}\label{lst:generated_unit_test_cases_java}
\end{listing}

==> Code/humanEval.tex <==
\begin{listing}[!ht]
{\renewcommand\theFancyVerbLine{%
\rmfamily\tiny\ifnum\value{FancyVerbLine}=25
  \setcounter{FancyVerbLine}{32}\ldots
\else
\arabic{FancyVerbLine}%
\fi
}
\begin{JavaSourceCode*}{label=\textcolor{black}{\tiny{TriangleArea.java}}}
package original;

class TriangleArea {
    /**
     * Given length of a side and high return 
     * area for a triangle.
     *
     * > triangleArea(5, 3)
     * 7.5
     * > triangleArea(2, 2)
     * 2.0
     * > triangleArea(10, 8)
     * 40.0
     */
    public static Double triangleArea(int a, int h) {
        return (a * h) / 2.0;
    }
}
\end{JavaSourceCode*}
}
\caption{Class Under Test from HumanEval}\label{lst:class_java}
\end{listing}

==> Code/humanEvalTest.tex <==
\begin{listing}[!ht]
{\renewcommand\theFancyVerbLine{%
\rmfamily\tiny\ifnum\value{FancyVerbLine}=25
  \setcounter{FancyVerbLine}{32}\ldots
\else
\arabic{FancyVerbLine}%
\fi
}
\begin{JavaSourceCode*}{label=\textcolor{black}{\tiny{TriangleAreaTest.java}},highlightlines={1-9}}
// TriangleAreaTest.java
package original;

import java.util.Arrays;
import java.util.Map;
import org.junit.jupiter.api.Test;
import static org.junit.jupiter.api.Assertions.*;

class TriangleAreaTest {
    @Test
	public void test1() throws Exception {
		assertEquals(7.5, original
                    .TriangleArea.triangleArea(5, 3));
	}

	@Test
	public void test2() throws Exception {
		assertEquals(2.0, original
                    .TriangleArea.triangleArea(2, 2));
	}

	@Test
	public void test3() throws Exception {
		assertEquals(40.0, original
                    .TriangleArea.triangleArea(10, 8));
	}
}
\end{JavaSourceCode*}
}
\caption{Test Class for Class Under Test from HumanEval}\label{lst:test_class_java}
\end{listing}

==> Code/sf110.tex <==
\begin{listing}[!ht]
{\renewcommand\theFancyVerbLine{%
\rmfamily\tiny\ifnum\value{FancyVerbLine}=25
  \setcounter{FancyVerbLine}{32}\ldots
\else
\arabic{FancyVerbLine}%
\fi
}
\begin{JavaSourceCode*}{label=\textcolor{black}{\tiny{JMenuHelper.java}}}
package visu.handball.moves.controller;

import java.awt.event.*;
import javax.swing.*;

public class JMenuHelper {
/**
	 * Add an element to the menubar.
	 * 
	 * @param menuBar a JMenuBar
	 * @param s a String
	 * 
	 * @return added JMenu
	 */
	public static JMenu addMenuBarItem(JMenuBar menuBar, String s) {
		JMenu menu;

		/**
		 * Suche nach '_' und nimm das nächste Zeichen als Mnemonic,
		 * sonst: normales Menu
		 */
		if (s.indexOf("_") > -1) {
			int pos = s.indexOf("_");
			char c = s.charAt(pos + 1);
			StringBuffer sb = new StringBuffer(s).delete(pos, pos + 1);
			menu = new JMenu(sb.toString());
			menu.setMnemonic(c);
		} else
			menu = new JMenu(s);

		menuBar.add(menu);
		return menu;
	}
 }
\end{JavaSourceCode*}
}
\caption{Class Under Test from Evosuite SF110 }\label{lst:class_java_sf110}
\end{listing}

==> Code/sf110Test.tex <==
\begin{listing}[!ht]
{\renewcommand\theFancyVerbLine{%
\rmfamily\tiny\ifnum\value{FancyVerbLine}=25
  \setcounter{FancyVerbLine}{32}\ldots
\else
\arabic{FancyVerbLine}%
\fi
}
\begin{JavaSourceCode*}{label=\textcolor{black}{\tiny{JMenuHelperTest.java}},highlightlines={1-15}}
// JMenuHelperTest.java
package visu.handball.moves.controller;

import java.awt.event.*;
import javax.swing.*;
import java.util.*;
import org.junit.jupiter.api.*;
import static org.junit.jupiter.api.Assertions.*;

/**
 * Test class of {@link JMenuHelper}.
 * It contains one unit test case for the 
 * {@link JMenuHelper#addMenuBarItem(JMenuBar, String)} method.
 */
class scenario3_JMenuHelper_addMenuBarItem_2000_10_Test {

    // Default Constructor
    scenario3_JMenuHelper_addMenuBarItem_2000_10_Test() {
        // Test code for a javax.swing component that implements event.
    }

    // Test methods for each of classes in this class.
    /**
     * Tests {@link JMenuHelper#addMenuBarItem(JMenuBar, String)}.
     */
    @Test
    public void testAddMenuItem() {
        assertNotSame(null, addMenuBarItem(null, ""));
        assertNotSame(null, addMenuBarItem(new JMenuBar(), ""));
        assertNotSame(null, addMenuBarItem("", ""));
    }
}
\end{JavaSourceCode*}
}
\caption{Test Class for Class Under Test from Evosuite SF110 }\label{lst:test_class_java_sf110}
\end{listing}

==> Code/tokenize_yaml.tex <==
\begin{PythonSourceCode*}{label=\tiny{typesystem/tokenizer/tokenize\_yaml.py},highlightlines={1-1}}
# create pytest function for validate_yaml
def test_validate_yaml(self):
    u = Uniqueness()
    assert u.make_hashable(True) == u.TRUE
    assert u.make_hashable(False) == u.FALSE
    assert u.make_hashable(1) == 1
    assert u.make_hashable(0.1) == 0.1
    assert u.make_hashable("a") == "a"
\end{PythonSourceCode*}

==> Files/ICPC/discussion_icpc.tex <==
\section{Discussion and Implications}\label{sec:discussion}
In this section, we discuss the results and provide the implications of the findings to practitioners and researchers.

\subsection{Implications of Having Code Descriptions and Sample Input-output}
% Code documentation is an important part of the software development process. It provides a clear and concise explanation of the code, making it easier for other developers to understand and work with. 
Code comments are considered the most important form of documentation for program comprehension beside the code itself \cite{Souza05}. 
% It can help to improve the quality and maintainability of the code. 
In our RQ1 findings, we observed that code comment could help with program comprehension but also help  provide more context to \pilot{} while generating unit tests. Adding the example input-output for a method can help the code generation model provide a more concise solution. To generate unit tests using a code generation model like GitHub Copilot, it is good to have code comments about having comparatively better coverage and passing unit tests, according to our study. However, our study shows that adding examples of input and output (which can be used as unit tests) can lead to more repetitive unit tests, even though the generated test cases can increase coverage. The more repetitive unit test does not increase the code coverage but are computationally time-consuming and need more human intervention to remove them, which can hinder productivity. Hence, it is better to add comments from comprehension tasks like unit test generation, but adding example input-output for test generation may lead to more repetitive unit tests.

\subsection{Unit Test Generation for Complex Software Projects}
Test case generation is the most labor-intensive task in software testing. Hence, there is a need for automated software test generation tools. However, they are particularly hard for a complex software system \cite{ANAND20131978}. One of the challenges of generating unit tests for complex software projects is that it can be difficult to identify the units that need to be tested. This is because complex software projects often consist of many interconnected components, and it can be difficult to isolate these components and test them individually. Another challenge is that complex software projects may have high variability, with many possible inputs and outputs. This can make it difficult to create unit tests that adequately cover all possible scenarios and ensure that the software works correctly.
Additionally, complex software projects may depend on external libraries or frameworks. This can make it difficult to create unit tests that accurately reflect the real-world conditions in which the software will be used, which can lead to test cases that are not reliable or effective. Our study investigates whether this problem could be solved with a program understanding model like Codex \cite{chen2021codex}. However, our work found that the code generation model needs a larger context window for the complex software system as it may not always be possible to infer data types, execution path \etc from the fine-tuned dataset and a small context window. One possible way is to fine-tune the model according to the code base to understand the context of the project.  However, it can be computationally hard and need to fine-tune regularly. Another way can be extending the context window size, but it may not be possible with the current system architecture for the large language model-based tool like GitHub Copilot. It is important to note that the generated unit tests may not be comprehensive or completely accurate, so you should review and verify the tests before using them in your testing process.

\subsection{Test Smells in the Generated Unit Tests}
In this section, we discussed the top three unit test smells found in the GitHub Copilot-generated unit tests.
\begin{itemize}[leftmargin=*]
    \item \textbf{Assertion Roulette} \cite{Simula.SE.525} occurs when multiple assertions exist in the same testing function without proper explanation. It can hamper the readability, understandability, and maintainability of the tests \cite{wajdi21} because it can be hard to understand for which assertion the test case fails. For example, this code is taken from the \textit{flutes} project where there is a test function for \code{ceil_div} in which there are three assertions without any explanation for each assertion. Hence, it is hard to understand what use of this assertion, and if it fails on any of them, it can be hard to explain.
    \begin{PythonSourceCode*}{label=\tiny{flutes/math.py}}
def ceil_div(a: int, b: int) -> int:
    r"""Integer division that rounds up."""
    return (a - 1) // b + 1
# create pytest function for ceil_div
def test_ceil_div():
    """Test ceil_div method."""
    assert ceil_div(1, 1) == 1
    assert ceil_div(1, 2) == 1
    assert ceil_div(2, 1) == 2
\end{PythonSourceCode*}
    \item A \textbf{magic number test} is a type of unit test that checks for the presence of so-called hard-coded numerical values that are used in the code without any explanation or context (``magic numbers'')~\cite{meszaros03}. 
    % For instance, a magic number might be a numerical constant that is used to represent a specific status or error code, or a value that is used as a threshold for comparison. 
    For instance, the following test has been taken from \textit{codetiming} project where this test the \code{stop} method. However, the test uses a hard-coded value, $0.1$, without any explanation. Since they are not explained or given a meaningful name, it can be difficult to know what they represent or why they are used in the code. Besides, if the value of the magic number needs to be changed, it can be difficult to find all instances of the magic number and update them.
\begin{PythonSourceCode*}{label=\tiny{codetiming/\_timer.py}}
# create pytest function for stop
def test_stop():
    """Test the stop method"""
    timer = Timer()
    timer.start()
    time.sleep(0.1)
    timer.stop()
    assert timer.last > 0.1
\end{PythonSourceCode*}
    \item A \textbf{duplicate assert} is an assertion in a unit test that is redundant or unnecessary. This can happen when a developer writes multiple assertions that test the same thing or when an assertion is included in the test even though it is already covered by another assertion \cite{peruma19}. The following example is taken from \textit{flutils} project, where the test case tests the conversion of a string with an underscore to the camel. However, in the test case, we can see it is testing the function with the same input \ie \code{'one_two_three'}. Duplicate asserts can be problematic because they can clutter the code and make it difficult to understand. They can also reduce the effectiveness of the tests because they may not provide any additional information about the code's behavior. 
\begin{PythonSourceCode*}{label=\tiny{flutils/strutils.py}}
# create pytest function for underscore_to_camel
def test_underscore_to_camel():
    """Test underscore_to_camel function."""
    assert underscore_to_camel('_one__two___') \
        == 'oneTwo'
    assert underscore_to_camel('one_two_three') \
        == 'oneTwoThree'
    assert underscore_to_camel('one_two_three') \
        == 'oneTwoThree'
\end{PythonSourceCode*}
%     \item \textbf{Exception handling} type test smell happens when there is exception handling in the test function \cite{peruma19}. It occurs when a test method explicitly a passing or failing of a test method is dependent on the production method throwing an exception \cite{wajdi21}. The following example is taken from \textit{semantic\_release} project where it uses exception handling in the test case and the assertion depends on that. Exception handling type test smell can be problematic because it can lead to incomplete or ineffective tests. It can also make it difficult to identify and fix errors in the code, because the tests are not catching the exceptions that are being thrown.
%     \begin{PythonSourceCode*}{label=\tiny{semantic\_release/ci\_checks.py}}
% # create pytest function for checker
% def test_checker():
%     @checker
%     def test():
%         assert False
%     try:
%         test()
%     except CiVerificationError:
%         assert True
%     else:
%         assert False
% \end{PythonSourceCode*}
%     \item \textbf{Conditional logic test} smell is a term used to describe a situation in which a unit test is overly complex or difficult to understand due to the use of conditional logic. This can happen when the test includes a large number of conditional statements, such as if-else statements or switch statements, which can make the test difficult to read and maintain \cite{meszaros03}. The following code is taken from \textit{flake8} where the code is branched with \code{with} multiple times. The use of conditional logic in tests can make the tests difficult to read and maintain, and can reduce their effectiveness. To avoid conditional logic test smell, it is important to keep your tests simple and easy to understand. Instead of using complex conditional statements, try to break the test down into smaller, simpler tests that each focus on a specific aspect of the code's behavior.
% \begin{PythonSourceCode*}{label=\tiny{flake8/main/git.py}}
% # create pytest function for copy_file_to
% def test_copy_file_to():
%     """Test copy_file_to method."""
%     with tempfile.TemporaryDirectory() as tempdir:
%         filename = "test.txt"
%         filepath = os.path.join(tempdir, filename)
%         contents = b"test"
%         with open(filepath, "wb") as fd:
%             fd.write(contents)
%         copy_file_to(tempdir, filepath, contents)
%         assert os.path.exists(filepath)
% \end{PythonSourceCode*}
\end{itemize}
% \subsection{Using LLM in Program Comprehension}

==> Files/ICPC/methodology_icpc.tex <==
\section{Methodology}\label{sec:method}


% In this section, we first introduce our research questions, and then 
% we detail our systematic process to answer each of them.



\input{Files/rquestions.tex}


\subsection{RQ1: Code Elements}

% of source code can have functions/procedures, modules, a class, or an individual method.

To answer this question, we performed three major steps: \textcircled{1} we collected Python and Java samples from the HumanEval dataset~\cite{chen2021codex} (and its extended version~\cite{2023multilingual}); \textcircled{2} we used \pilot{} to generate unit tests; \textcircled{3} we compute the line/branch coverage for the  unit tests and the total number of unique and correct generated unit tests. These steps are detailed below.


\subsubsection{\textbf{Data Collection}}\label{subsec:dataset}
% In this question, we investigate the influence of functionality description and examples of input-output in the prompt during unit test generation. 
First, we retrieved samples from the \textbf{HumanEval dataset}~\cite{chen2021codex} and its \textbf{extended version} created by the AWS AI Labs \cite{2023multilingual}. We use the HumanEval dataset and its extended version because they have been widely used in prior works to evaluate large language models trained on code \cite{Nijkamp2022ACP, incoder, gpt-code-clippy, siddiq2022empirical}.

The HumanEval dataset consists of 164 \textbf{\textit{prompts}} and their \textbf{\textit{canonical solution}} written in \textbf{Python}~\cite{chen2021codex}. 
For example,  the sample shown in \listref{lst:filter_integers} is taken from the HumanEval dataset\footnote{The code formatting is modified for a better presentation.}. This sample contains a \textit{prompt} (lines 1--11) and its \textit{canonical solution} (line 12). The \code{filter_integers(values)} function takes as a parameter a list of objects and returns a new list that includes only the integers from the \code{values} list. As depicted in this figure, the prompt  includes different code elements. It contains \textit{import statements}, the \textit{function signature}, a docstring with the function's \textit{description}, and \textit{input-output} examples. The sample also includes the function implementation (\ie the canonical solution for the prompt).

\input{Code/filter_integers.tex}



The extended version of HumanEval~\cite{2023multilingual} provides \textbf{160} \textbf{prompts}, crafted from the original Python-based HumanEval dataset~\cite{chen2021codex} for Java and other programming languages. However, this extended version does not provide a function implementation for each prompt (\ie  canonical solution). Hence, we wrote the solution ourselves and tested our implementation using the provided test cases for the prompt~\cite{2023multilingual}. The canonical solution is encapsulated in a class as a \codeJava{public} and \codeJava{static} method, whereas the prompt is a Javadoc for the method. \listref{lst:truncatenumber} shows a sample taken from the extended HumanEval dataset\footnote{The code formatting is modified for a better presentation.}, where the prompt is highlighted in blue, and the canonical solution is  in lines 15--18.

\input{Code/TruncateNumber.tex}
% In that way, we have 160 functionally correct samples for Java for this research question.
% we followed the approach described by the AWS AI Labs in their paper \cite{2023multilingual}\joanna{you followed the approach to do what?}. We used the \pilot{} to generate solutions from the Java-based prompts and see if they passed the provided test cases. \pilot{} provides up to 10 additional solutions. Until the solution passed the test cases, we tried them one by one. If we can not find a solution by GitHub Copilot, we wrote the solution on our own and tested with the provided unit tests in the dataset \cite{2023multilingual}. In that way, we have 160 functionally correct samples for Java for this research question.


Therefore, we combine the prompts and their respective canonical solution from the HumanEval dataset and compile them into \textbf{164 Python samples}. Similarly, we combine the \textbf{160} prompts from the extended HumanEval dataset and our canonical solutions and compile them into \textbf{160 Java samples}. Subsequently, we created three different \textit{unit testing scenarios} to investigate how the code elements of a unit influence the generated test cases. To create these scenarios, we modified each of these samples in the following ways:
\begin{itemize}[leftmargin=*]
    \item \underline{\textbf{Scenario 1:}} The samples only contain the \textit{import statements},  function's \textit{signature} and \textit{implementation}. For instance, these are lines \textbf{1} to \textbf{3} and \textbf{12} in \listref{lst:filter_integers}.
    \item \underline{\textbf{Scenario 2:}} The samples include the function's \textit{signature}, \textit{implementation} and a docstring with the function's \textit{description} but excluding the  input-output examples. For example, in the sample from \listref{lst:filter_integers} the new sample would only contain lines \textbf{1} to \textbf{6}, \textbf{11} and \textbf{12}. 
    \item \underline{\textbf{Scenario 3:}} We use the original sample without excluding anything, \eg the  code in \listref{lst:filter_integers} would be used as it is.
\end{itemize}

Scenarios 1 and 2 aim to investigate whether Copilot is useful in helping engineers to follow a Test-Driven Development (TDD)~\cite{beck2003TDD}, where test cases are written before the actual code implementation. Scenario 3 models a case where tests are written after the actual unit under test.
At the end of this first step, we obtained a total of \textbf{492} samples for Python (\ie \textbf{164} samples in each scenario) and \textbf{480} samples for Java (\ie \textbf{160} samples in each scenario).



\subsubsection{\textbf{Unit Test Generation}}

We generate unit tests by following a two-step process. First, we ask \pilot{} to generate framework-agnostic test cases (\ie sample input-output pairs). Second, we instruct \pilot{} to generate a unit test using an existing framework. These steps are detailed below:


\begin{itemize}[leftmargin=*]
    \item[--] \textbf{\textit{Input-Output Generation}}: We append to each of the \textbf{492} Python samples the following code comment: \code{# Create 10 test cases for the above function}.  This code comment instructs \pilot{} to generate  framework-agnostic test cases (\ie sample input-output pairs) using the sample function as a \textit{context} for code generation. This way, we have a total of \textbf{1,640} test cases (164 $\times$ 10) for each scenario. For example, the code snippet in \listref{lst:generated_test_cases} shows the line added to the code in \listref{lst:filter_integers} (highlighted) and the test cases generated by \pilot{} (lines 14--25). We can see that \pilot{} generates test cases as an \texttt{array} of \texttt{tuples}. The tuple's first element  is the \textit{input}, and the tuple's second element is the expected \textit{output} for the given input.
    We can also see that any testing framework can iterate these input-output pairs, for example, \texttt{unittest}\footnote{\url{https://docs.python.org/3/library/unittest.html}}, \texttt{pytest}\footnote{\url{https://docs.pytest.org/en/7.2.x/}} \etc
% 
\input{Code/generated_test_cases_python.tex}
Similarly, for the \textbf{480} Java samples, 
we append to it  the following code comment: \codeJava{// Create 10 test cases for the above method}. The code comment instructs \pilot{} to generate framework-agnostic test cases using the method (and its JavaDoc, if any) as context. For Java, the generated list of input-output pairs is an \codeJava{ArrayList} of object arrays. The last array element indicates the possible output of the solution method, where the rest of the elements in the object array are the input. For example, the code snippet in \listref{lst:generated_test_cases_java} shows the line added to the code in \listref{lst:truncatenumber} (highlighted) within the class and the test cases generated by \pilot{} (lines 20--34). Except for the last element in the object array, the remaining elements are input for the targeted method (\ie \codeJava{truncateNumber}). The last element is the projected output from the method. As this list is framework-agnostic, they can be tested with any testing framework for Java, for example, \texttt{JUnit}\footnote{\url{https://junit.org/junit5/docs/5.8.1/api/index.html}}.

\input{Code/generated_test_cases_java.tex}
    \item[--] \textbf{\textit{Test Functions/Methods Generation}}: For the Python samples, we add a code comment (``\texttt{\# write pytest functions using the test\_Ccases array}'') after the test case array to generate the unit tests using \texttt{pytest}, a testing framework for Python. Sometimes, we also need to provide the function name as an additional prompt such as ``\code{def test_answer_0():}'' to provide more context to the GitHub Copilot. For the Java samples, we add this code comment: \texttt{// write JUnit functions using the test\_Cases array} after the test case list to generate unit tests implemented using \texttt{JUnit}, a Java unit test framework. As like Python, we might give additional prompts in the newline for Java, like this: \codeJava{@Test public void test_0()}.
    
    As our work focuses on unit tests, we do not change anything in the unit test array if there is anything wrong. However, in the generated testing functions for \texttt{pytest} and \texttt{JUnit}, we manually check them, and we need to edit or rewrite the functions if there is any error.

For instance, the code in \listref{lst:generated_unit_test_cases} shows the lines added to the \textit{filter\_integers.py} sample  (highlighted) and the  testing functions generated by \pilot{} (lines 28 and beyond).  Due to space constraints, we only present the first 3 testing functions instead of 10. We can see that in the first testing function, it executes the \texttt{filter\_integers} by taking the input of the first element of the tuple from the test case array, and then, after collecting the result, it uses \texttt{assert} to check the correctness of the result.

\input{Code/generated_unit_tests.tex}

The code in \listref{lst:generated_unit_test_cases_java} shows the lines added to the \textit{TruncateNumber.java} sample  (highlighted) and the  testing functions generated by \pilot{} (lines 28 and beyond). The first testing function executes the \texttt{truncateNumber} by taking the input of the first element of the tuple from the test case array. Then, after collecting the result, it uses \texttt{assert} to check the correctness of the result.

\input{Code/generated_unit_tests_java.tex}

As our work focuses on unit tests, we do not change anything in the unit test array if there is anything wrong. However, in the generated testing functions for \texttt{pytest} and \texttt{JUnit}, we manually check them, and we need to edit or rewrite the functions if there is any error.
\end{itemize}

\subsubsection{\textbf{Data Analysis}}

Once we generate all the unit tests for all the functions in each scenario, we use \texttt{pytest}  testing framework and \texttt{Coverage.py} \footnote{\url{https://coverage.readthedocs.io/en/6.5.0/}} for Python and \texttt{JUnit}  testing framework and coverage feature from IntelliJ IDEA IDE \footnote{\url{https://www.jetbrains.com/idea/}} to  compute the following metrics: line coverage, branch coverage, test correctness, and test repetition. These metrics are defined as follows:

\begin{itemize}[leftmargin=*]
    \item \textbf{Line Coverage} is a common metric to measure the performance of a software tester \cite{codecoveragegoogle,michael18}. This metric calculates how many lines have been executed by the unit tests out of the total number of lines, as follows: 
    \begin{equation}\centering\small
    \text{Line Coverage} = \frac{Number~of~executed~lines}{Total~number~of~lines} \times 100
    \end{equation}
    For instance, if a function has 20 lines and only 15 lines are executed using the generated unit tests, then the line coverage of these unit tests will be 75\%.
    \item \textbf{Branch Coverage} is the most well-known and practiced metric in software testing \cite{codecoveragegoogle}. A branch occurs due to conditional statements, such as \texttt{if} conditions, \texttt{loops}, \texttt{switch} cases \etc~In this case,  the program's execution follows different parts of the source code. A good set of unit tests should cover all the branches. The branch coverage of a unit test is computed as:
    \begin{equation}\centering\small
        \text{Branch Coverage}= \frac{Number~of~visited~branches}{Total~number~of~branches} \times 100
    \end{equation}
    For example, if a function has 8 branches and the unit tests visit 5 of them, the branch coverage of these unit tests will be 62.5\%.
    
    \item \textbf{Test Correctness} aims to measure how effectively \pilot{} generated correct unit tests. Since the canonical solution on the HumanEval dataset and its extended version \cite{chen2021codex, 2023multilingual} is a correct implementation, a test case generated by Copilot should not fail. Thus, we compute the number of GitHub Copilot-generated unit tests that passed while testing the canonical solutions as means to find the correctly generated unit tests.

    \item \textbf{Duplicate Test} means that two (or more) unit tests have the same input-output pairs in the generated test cases \cite{peruma19}. Duplicate tests do not increase the coverage but take additional computational power to generate and execute. Hence, we report the number of samples for which \pilot{} generated duplicate tests.
    
    % Finally, we calculate the number of test correctness and repetitive unit tests. Usually, in the software development life cycle, unit tests should be written after having the requirement and before writing the actual code \latif{citation needed}. However, in our case, especially for the first research question, we performed a controlled experiment where the correctness of the codes was already vetted by the creator of the HumanEval dataset \cite{chen21 }and the other peers who used this dataset\latif{citation needed}. Hence, if the unit test is functionally correct, it should not fail ideally for a sample in the HumanEval dataset. For this reason, we calculate the number of GitHub Copilot-generated unit tests that failed. We also calculate the number of repetitive unit tests as they do not increase the coverage but affect the cost of generating and checking them.
\end{itemize}




\subsection{RQ2: Comparison with Pynguin}
In this second question, we compare the Python unit tests generated by \pilot{} with Pynguin, a state-of-the-art approach~\cite{pynguinjournal,lukasczyk2022pynguin}. Pynguin is an open-source state-of-the-art automated test generation framework for \textbf{Python}. Given a Python module and its dependencies as input, Pynguin generates unit tests. 

To answer RQ2, we \textcircled{1}  retrieve open source Python modules previously used to evaluate Pynguin; \textcircled{2} use Pynguin and \pilot{} to generate unit tests for these modules; and \textcircled{3} compute branch coverage metrics for the generated unit tests. Each of these steps are described in the next subsections.

\subsubsection{\textbf{Data Collection}}

We performed the following steps to collect the dataset for this research question:
\begin{enumerate}[leftmargin=*]
    \item \textbf{Initial dataset collection}: Prior work empirically evaluated Pynguin \cite{pynguinjournal} using 170 modules from 24 open source Python projects. Out of these 170 modules, we exclude 36 modules from 12 projects as Pynguin did not produce any result for these modules. Since we aim to compare the effectiveness of \pilot{} with Pynguin, we only focus on the modules in which Pynguin can generate unit tests. After excluding these modules, we had 134 modules from 22 projects in this first step.
    \item \textbf{Exclusion before running coverage tool:} Next, we use \pilot{} to generate unit tests for standalone functions with \code{return}  statement. Hence,  we excluded 84 modules from 15 projects that did not have any standalone function with a \code{return} statement. We discard these modules because they cannot be tested with an \texttt{assert}-based unit test.    
    
    \item \textbf{Exclusion after running coverage tool}:  When we run the tool (\ie \code{Coverage.py}) to have the metrics for evaluation, the test cases may \textit{pass}, \textit{fail}, or run into an \textit{error}. When all the unit tests for a module run into an error, we exclude them from the result. We excluded 13 modules from 6 projects during this step.
\end{enumerate}

As a result, we obtained \textbf{37} modules from \textbf{14} projects to generate unit tests by \pilot{} and Pynguin.
% \tblref{tab:projectlist} presents the project list with their version and the number of modules we used in our study.


% \input{Tables/project_list.tex}

\subsubsection{\textbf{Unit Test Generation}}
% We use a testing framework-agnostic approach for the first research question, but for the second research question, we directly generate testing functions targeting \texttt{pytest} .  

To generate Python unit tests using \pilot{}, we add the following code comment after the targeted method: \texttt{\# create pytest function for \{method name\}}. This prompt instructs \pilot{} to generated testing functions using the function under test as context.
The following example is taken from the \textit{``typesystem''} repository and the \textit{tokenize\_yaml.py} file. After the \code{validate_yaml()} method, we asked \pilot{} to generate \code{pytest} testing functions, and it generates unit tests for the \texttt{make\_hashable} function of the \texttt{Uniqueness} class. 
% The example is slightly modified for a better presentation.


\input{Code/tokenize_yaml.tex}

However, as in the previous example, it can be seen that it has \texttt{self} keyword in the function parameter, and as this method is not part of a Python class, it can cause an error. We remove this \texttt{self} keyword from the parameter to make it workable with the testing tool. We take only this corrective approach on the generated test cases by GitHub Copilot. We generate \textbf{162} unit tests for these 37 modules from 14 open-source projects.

\subsubsection{\textbf{Data Analysis}}
We compare our result with Pynguin \cite{pynguinjournal}, which reports their branch coverage. However, in our result, we report not only branch coverage but also line coverage. We also report the number of generated unit tests that passed for each project.

\subsection{RQ3: Test Smells}
Unit tests, just like regular  code, need to be understood and maintained by developers \cite{zampetti2020demystifying}. Thus, automatically generated test cases must be not only correct, but also free of quality problems. In this question, we aim to understand the \textit{quality} of the generated unit tests  by investigating the presence of test smells.

\subsubsection{\textbf{Test Smell Selection}}
The literature have discussed common test smells that can arise in unit tests written in Python~\cite{pynose, Simula.SE.525, peruma19, meszaros03, greiler13, daniel21, wajdi21, peruma19}. In our study, we focus on the same 9 test smells that were used to evaluate Pytest-smell \cite{pytest_smell}, a test smell detection tool for Python. These 9 test smells are: Assertion Roulette (AR), Conditional Logic Test (CLT), Duplicate Assert (DA), Exception Handling (EH), Eager Test (EA), Magic Number Test (MNT), Redundant Print (RP), Sleepy Test (ST) and Unknown Test (UT).  
We choose to focus on these 9 test smells because prior work \cite{pytest_smell} investigated the distribution of these test smells in three open-source projects and they are very prevalent in the human-written unit tests. For example, at least 10\% tests in these three open-source projects contain Assertion Roulette (AR), Magic Number Test (MNT), Conditional Logic Test (CLT), Duplicate Assert (DA). Hence, we can compare whether the distribution of the test smells in the generated unit tests follow similar trend as human-written smells in the open-source projects. 
\tblref{tab:test-smell} summarizes the 9 test smells with description and the source.
\input{Tables/smells.tex}

% % To answer this question, we first need to understand what are the common test smells that can arise in unit tests written in Python.
% %for evaluating Pytest-smell \cite{pytest_smell}, a test smell detection tool for Python, its author collected a dataset from three open-source projects: Pillow \cite{pillow}, Sanic \cite{sanic}, and Flask \cite{flask}. The distribution of the test smells in the unit tests of these projects followed this: Assertion Roulette, Magic Number Test, Conditional Logic Test, Duplicate Assert, Unknown Test, Exception Handling, Eager Test, Sleepy Test, and Redundant Print. Thus, for \textbf{RQ3}, we focused on these 9 test smells. We tried to investigate if an AI-based assistant tool like \pilot{} can mimic the same test smells in the same distribution. In Table \ref{tab:test-smell}, we summarize this investigated test smells including their description. 

\subsubsection{\textbf{Dataset and Result Processing}}
We use \textbf{162} unit tests for the 37 modules from 14 open-source projects generated by \pilot{} in the previous research question (RQ2). We manually go through the generated unit tests to find out the test smells as we can not run any detection tool (\ie Pytest-smell \cite{pytest_smell}). Our unit test generation process for RQ2 is not standard \ie test cases not in a standalone test file. Consequently, these static rules-based test smell detectors can not find the test cases in the usual Python file and hence no test-smell detection.

% \joanna{why haven't we put the unit test code in a separate file and then used the tools?}


% to detect the unit test smells in Python. 
% This tool can detect 9 test smells: Assertion Roulette, Magic Number Test, Conditional Logic Test, Duplicate Assert, Unknown Test, Exception Handling, Eager Test, Sleepy Test, and Redundant Print. \tblref{tab:test-smell} shows these investigated test smells including their description, their detection tools as well as the original study that described the test smell. 
% To do an empirical evaluation, the work focused on nine test smells. The distribution of the dataset for the empirical evaluation was collected from three open-source projects: Pillow \cite{pillow}, Sanic \cite{sanic}, and Flask \cite{flask}. The distribution of the test smells in the unit tests of these projects followed this: Assertion Roulette, Magic Number Test, Conditional Logic Test, Duplicate Assert, Unknown Test, Exception Handling, Eager Test, Sleepy Test, and Redundant Print.
% Thus, for \textbf{RQ3}, we focused on these 9 test smells. We tried to investigate if the AI based assistant tool like \pilot{} can mimic the same test smells in the same distribution. In Table \ref{tab:test-smell}, we summarize these investigated test smells including their description, their detection tools as well as the original study that described the test smell. 


% we collect the possible test smells, especially for Python, from the work of Fernandes \etal \cite{daniel21}. This prior work made comprehensive lists of 20 test smells focusing on Python and announced four new test smell types. Then, we checked three test smells detection tools for Python: PyNose \cite{pynose}, Pytest-Smell \cite{pytest_smell} and TEMPY \cite{tempy}. In these tools, we find three additional test smells they can detect. In our study, we focus on 8 test smells that can be detected by two or more tools: Assertion Roulette (AR), Conditional Logic Test (CLT), Duplicate Assert (DA), Exception Handling (EH), Magic Number Test (MNT), Redundant Print (RP), Sleepy Test (ST) and Unknown Test (UT). In Table \ref{tab:test-smell}, we summarize the 27 test smells with description and their detection tools.




% \joanna{now what? @Lati: can you please clarify? There are 9 test smells. My assumption is that we run PytestSmell on a set of unit tests generated by Copilot, what unit tests are these? Are these from RQ`1? RQ2? Or something else? Please add.}

\subsubsection{\textbf{Data Analysis}}
We calculate the weighted average ($W$) of the unit tests with test smells for each test smell type and project using this formula ($m$ is the number of modules): 
\begin{equation}
    W = \frac{\sum_{n=1}^{m} Percentage~of~Tests~with~Smell}{ \sum_{i=1}^{m} Y_i}
\end{equation}

In this formula, we accumulate the \textit{percentage of unit tests with test smells} and then divide by the sum of $Y_i$, which is defined as:


\[ Y_i =
 \begin{cases}
    0, & Module~not~Containing~Smell \\
    1, & Module~Containing~Smell 
  \end{cases}
\]
 Simply put, $Y_i$ is a function that returns \textit{one} if any of the unit tests in the module contains the particular test smell and \textit{zero} if the module is not containing the particular test smell. Now, if there is no module with smell, we consider that the weighted average ($W$) is \textit{zero}.
 
 For example, we have five modules and the unit tests in each module contains 30\%, 15\%, 0\%, 25\%, 12\% magic number unit test (MNT) smell respectively. Then, the weighted average ($W$) for MNT will be, $\frac{(30\% + 15\% + 25\% + 12\%)}{4} = 20.5\%$. We remove the value of the third module as it is not containing any smell.

 %The formula for 

\begin{comment}

\subsection{Tools}
We use the following tools in our work:
\begin{itemize}
    \item \texttt{pytest}  is a well-known testing framework for Python. It was first introduced in late 2002. It can be used to create a variety of software tests, including functional, end-to-end, unit, and integration tests. Its features include fixtures, assert re-writing, and parameterized testing. We use version 6.2.5 and its unit-testing functionality to evaluate the generated unit tests by GitHub Copilot.
    \item Python projects can have their code coverage evaluated using the utility \texttt{Coverage.py}. It keeps track of the code segments executed in your program while monitoring it; then, it examines the source code to find segments that should have been performed but weren't. In our work, we use the 6.5.0 version of this tool with \texttt{pytest} to calculate line and branch coverage.
    \item \texttt{JUnit}  is a popular Java-based unit testing framework used to test the functionality of individual units of code.
    With JUnit, the developers can write test cases that define the expected behavior of the code and automatically run those test cases to ensure that the code is correct. In our work, we use JUnit 5.8.1 API in the IntelliJ IDE for Java \cite{jetbrain}.
\end{itemize}
\end{comment}

==> Files/ICPC/methodology_old.tex <==
\section{Methodology}\label{sec:method}

Figure~\ref{fig:overview} shows an overview of the steps we performed in our study to answer our research questions. The next subsections detail each of those steps.


\subsection{Data Collection}\label{subsec:dataset}

\subsubsection{RQ1: Prompt elements}
To answer \textbf{RQ1}, we used the HumanEval dataset \cite{chen2021codex} to demonstrate the correlation with unit test generation and the presence of functionality description and examples of input-output in prompt. We chose to use HumanEval because this dataset has been used in prior works to evaluate large language models trained on code \hl{citations}.

The HumanEval dataset consists of 164 \textbf{\textit{prompts}} and their \textbf{\textit{canonical solutions}} written in Python. 
% These prompts include different elements, such as import statements, the function's signature and description as well as input-output examples to provide more context to the code generation model. 
% The prompts from the dataset are given as input to the code generation model. Then, the code generation model generates code by taking context from the input prompt. The functional correction of the generated code from the code generation model is checked with an execution-based approach with unit test cases. Hence, the dataset also contains the unit tests for each prompt to check the generated code's functionality. 
For example,  the sample shown in \figref{fig:filter_integers} is taken from the HumanEval dataset\footnote{The code formatting is modified for a better presentation.}. The \code{filter_integers(values)} function takes as a parameter a list of objects and returns a new list that includes only the integers from the \code{values} list. The prompt (lines \textbf{1} to \textbf{11}) includes \textit{import statements}, the \textit{function signature}, a docstring describing the method's \textit{functionality}, and \textit{input-output} examples to be provided to a code generation model. The sample also includes the function implementation (\ie the canonical solution for the prompt).

\input{Code/filter_integers.tex}


For this question, we first collect the prompts and their respective canonical solution from the HumanEval dataset and compiled into 164 samples. Subsequently, we created three different scenarios to investigate how elements of a prompt influence the generated test cases. To create these scenarios, we modified each of these samples in the following ways:
\begin{itemize}[leftmargin=*]
    \item \underline{\textbf{Scenario 1:}} The samples only contain the \textit{function signature} and \textit{functional code}. For instance, these are lines \textbf{1} to \textbf{3} and \textbf{13} in the previous example (\code{filter_integers.py}).
    \item \underline{\textbf{Scenario 2:}} The samples include the \textit{function signature} as well as a docstring with the description of the method's \textit{functionality} but exclude the  input-output examples in the code comment. For example, in the sample from \figref{fig:filter_integers} the new sample would only contain lines \textbf{1} to \textbf{6}, \textbf{11} and \textbf{12}. 
    \item \underline{\textbf{Scenario 3:}} We use the original sample without excluding anything, \eg the above code would be used as it is.
\end{itemize}

Scenarios 1 and 2 aim to investigate whether Copilot is useful in helping engineers to follow a Test-Driven Development (TDD)~\cite{beck2003TDD}, where test cases are written prior to the actual code implementation. Scenario 3 models a case where tests are written after the actual unit under test.



\subsubsection{RQ2: Test Smells in the Generated Unit Tets}
Alexandru Bodea created Pytest-smell \cite{pytest_smell} to detect the unit test smells in Python. To do an empirical evaluation, the work focused on nine test smells. The distribution of the dataset for the empirical evaluation was collected from three open-source projects: Pillow \cite{pillow}, Sanic \cite{sanic}, and Flask \cite{flask}. The distribution of the test smells in the unit tests of these projects followed this: Assertion Roulette, Magic Number Test, Conditional Logic Test, Duplicate Assert, Unknown Test, Exception Handling, Eager Test, Sleepy Test, and Redundant Print.

For \textbf{RQ2}, we focused on these 9 test smells. We tried to investigate if the AI based assistant tool like GitHub Copilot can mimic the same test smells in the same distribution. In Table \ref{tab:test-smell}, we summarize these investigated test smells including their description, their detection tools as well as the original study that described the test smell. 


% we collect the possible test smells, especially for Python, from the work of Fernandes \etal \cite{daniel21}. This prior work made comprehensive lists of 20 test smells focusing on Python and announced four new test smell types. Then, we checked three test smells detection tools for Python: PyNose \cite{pynose}, Pytest-Smell \cite{pytest_smell} and TEMPY \cite{tempy}. In these tools, we find three additional test smells they can detect. In our study, we focus on 8 test smells that can be detected by two or more tools: Assertion Roulette (AR), Conditional Logic Test (CLT), Duplicate Assert (DA), Exception Handling (EH), Magic Number Test (MNT), Redundant Print (RP), Sleepy Test (ST) and Unknown Test (UT). In Table \ref{tab:test-smell}, we summarize the 27 test smells with description and their detection tools.

\input{Tables/smells.tex}



\subsubsection{RQ3: Comparison with the SOTA}
For \textbf{RQ3}, we use the samples used to empirically evaluate the Pynguin tool \cite{pynguinjournal}, which is a state-of-the-art approach to generate unit test cases. This prior work used 170 \hl{python} modules from 20 open source projects in their evaluation. However, 32 out of 170 modules do not produce any result by their tool, so we do not include them in our study \joanna{this might be questioned. It would still be worth it to compare the cases where pyguin did poorly, but Copilot could doo it}. In addition, if there are no functions in the module with a \texttt{return} statement, they can not be tested with \texttt{assert}-based unit test. Hence, we also exclude these modules. Finally, if there are methods as part of the class, we exclude them from our study \joanna{we should not exclude methods!}. 


\joanna{We should just say: we investigate 138 projects. The explanation below should be a finding placed on the results section. We should describe as a result/observation. Remember the goal is not defend copilot, but to show its strength and weaknesses in unit test generation}

\textcolor{brown}{Open-source projects  have lots of intra- and inter-dependencies among different modules. Though GitHub Copilot can work with publicly available common libraries, it may not be easy to infer output from the custom datatype and class declaration, which can be essential to test a function. According to the GitHub Copilot FAQ web page\cite{copilot}, GitHub Copilot collects ``code snippets'', which include  source code that the users are editing, related files and other files open in the same IDE or editor, URLs of repositories, and files path. However, it has a context window to inference output; for example, in the GPT-3 playground from OpenAI \cite{playgorund}, it uses 2,048 tokens for the combined prompt and the resulting generated completion. Though the GitHub Copilot does not mention the context window size, it is hard for the current system architecture to accommodate a large window. Hence, it may not be enough to generate a correct unit test for a complex project with many dependencies.
For this reason, we try to generate unit tests for every function in the 138 modules with return statements. Still, if we run into errors for every test case for a particular module in the result generation part, we exclude them. This way, we have 40 modules from 15 projects with at least one passed or failed test unit test case. In Table \ref{tab:projectlist}, we present the project list with their version and the number of modules we use in our work.}
\begin{table}[ht!]
\centering
\caption{Project List with Their Version}
\label{tab:projectlist}
% \resizebox{0.75\columnwidth}{!}{%

\begin{tabular}{|l| c|c|}\hline
\textbf{Project Name} & \textbf{Version}& \textbf{Number of Modules} \\\hline
apimd & 1.2.1 0& 1\\
codetiming & 1.3.0 & 1\\
flake8 & 3.9.0& 3 \\
flutes & 0.3.0& 1 \\
flutils & 0.7& 3 \\
httpie & 2.4.0& 4 \\
isort & 5.8.0 & 2\\
pdir2 & 0.3.2& 4 \\
py-backwards & 0.7& 4 \\
python-string-utils & 1.0.0& 2\\
python-semantic-release & 7.15.3& 3\\
pytutils & 0.4.1& 5 \\
sty & 1.0.0rc1 & 1\\
thonny & 3.3.6 & 4\\
typesystem & 0.2.4& 2\\\hline
\end{tabular}
% }
\end{table}





\subsection{Unit Test Generation}


In this part, we prompt the GitHub Copilot to generate unit tests. We add this comment to the code from three scenarios described in the previous section: \texttt{\# Create 10 test cases for the above function}. Then, GitHub Copilot generates test sets. However, sometimes GitHub Copilot does not generate test cases with only one edit action (\ie pressing enter after the comment); we have to provoke the GitHub Copilot by doing additional edit actions to generate 10 test cases. We intend these unit tests are Python testing \textbf{framework-agnostic}. This way, we have $1,640(164\times 10)$ unit tests for each scenario.

The following code is an extension of the previous code in Section \ref{subsec:dataset}. We highlight the additional prompt in line no 1. We present three test cases instead of 10 for a better presentation. We can see that GitHub Copilot generates test cases as an \texttt{array} of \texttt{tuples}. For this example, the first element of the first tuple in the array will be the input, and the second element of the tuple should be the method's output for the given input.
We can also see that any testing framework can use these unit tests, for example, \texttt{unittest} \cite{unittest}, \texttt{pytest} \cite{pytest} \etc
\begin{PythonSourceCode*}{label=\tiny{filter\_integers.py},highlightlines={1-1}}
# Create 10 test cases
test_cases = [
    (['a', 3.14, 5], [5]),
    ([1, 2, 3, 'abc', {}, []], [1, 2, 3]),
    ([1, 2, 3, 'abc', {}, [], 'def'], [1, 2, 3]),
 ]
\end{PythonSourceCode*}

We use a testing framework-agnostic approach for the first research question, but for the second research question, we directly generate testing functions targeting \texttt{pytest} \cite{pytest}. In addition, we only focus on the methods in the module which have \texttt{return} statement so that they can be validated with \texttt{assert} based unit tests. To generate unit tests using GitHub Copilot, we provide the prompt in this format after the targeted method: \texttt{\# create pytest function for \{method name\}}. Sometimes, we need to give more context in the prompt like  \texttt{def test\_\{method name\}}. We stop invoking edit actions for this research question until we receive at least one unit test from the GitHub Copilot. Our unit test creation method is not ideal, as they are present after each method and in the same file. This way is done to provide the GitHub Copilot with more related context, as discussed before. Hence, we keep the unit test generation prompt after the targeted method to provide more recent context.


% COPARISON WITH PYNGUIn

The following example is taken from the "typesystem`` repository and tokenize\_yaml.py file. After the \texttt{validate\_yaml} method, we asked GitHub Copilot to generate \texttt{pytest} testing functions, and it generates unit tests for the \texttt{make\_hashable} function of the \texttt{Uniqueness} class. The example is slightly modified for a better presentation.
\begin{PythonSourceCode*}{label=\tiny{typesystem/tokenizer/tokenize\_yaml.py},highlightlines={1-1}}
# create pytest function for validate_yaml
def test_validate_yaml():
    u = Uniqueness()
    assert u.make_hashable(True) == u.TRUE
    assert u.make_hashable(False) == u.FALSE
    assert u.make_hashable(1) == 1
    assert u.make_hashable(0.1) == 0.1
    assert u.make_hashable("a") == "a"
\end{PythonSourceCode*}
However, as in the previous example, it can be seen that it has \texttt{self} keyword in the function parameter, and as this method is not part of a Python class, it can cause an error. We remove this \texttt{self} keyword from the parameter to make it workable with the testing tool. We take only this corrective approach on the generated test cases by GitHub Copilot.

\subsection{Result Processing}

In the previous section, we describe how we generate unit tests by GitHub Copilot, and they are framework agnostic. However, to evaluate, we use \texttt{pytest} \cite{pytest} testing framework, and \texttt{Coverage.py} \cite{coverage} to measure different metrics. We will briefly introduce these tools in the next section.

To calculate evaluation metrics, we first need to generate testing functions for \texttt{pytest} from the previously created \texttt{test\_cases} array described in the last section. Instead of manually crafting the testing functions, we semi-automated the process with the help of GitHub Copilot. After the array containing unit tests, we provide this comment to generate test functions: \texttt{\# write pytest functions using the test\_cases array}. Sometimes, we also need to provide the function name as an additional prompt such as \texttt{def test\_answer\_0():} to provide more context to the GitHub Copilot. As our work focuses on unit tests, we do not change anything in the unit test array if there is anything wrong. However, in the generated testing functions for \texttt{pytest}, we manually check them and need to edit or rewrite the functions if there is any error. 

In the following code, we can see the generated testing functions by GitHub Copilot. We highlight the prompt added after the demonstrative example in the previous section. We only present the first three testing functions instead of 10 for a better presentation. We can see that in the first testing function, it executes the \texttt{filter\_integers} by taking the input of the first element of the tuple from the test case array, and then, after collecting the result, it uses \texttt{assert} to check the correctness of the result.
\begin{PythonSourceCode*}{label=\tiny{filter\_integers.py},highlightlines={1-1}}
# write test functions
def test_answer_0():
    result = filter_integers(test_cases[0][0])
    assert result == test_cases[0][1]

def test_answer_1():
    result = filter_integers(test_cases[1][0])
    assert result == test_cases[1][1]

def test_answer_2():
    result = filter_integers(test_cases[2][0])
    assert result == test_cases[2][1]
\end{PythonSourceCode*}
Then, we use \texttt{pytest} \cite{pytest} testing framework and \texttt{Coverage.py} \cite{coverage} to calculate the metrics. 

We do not need to process anything for the second research question as it is not a framework-agnostic approach. Hence, we directly calculate the metrics described in the next section. We also use these GitHub Copilot-generated unit tests for the project modules for finding test smells to answer the last research question. We manually go through the project test cases and check whether there are any test smells.


We do not use the generated unit tests from the different scenarios using the HumanEval dataset because, for this case, we create a testing-framework agnostic input-output list that any framework can later use. Also, we use \texttt{pytest} \cite{pytest} for this task and correct them manually if anything is wrong. Hence, it uses GitHub Copilot to generate unit tests, taking help to generate testing functions, but relying on human involvement affects generating test smells. For example, there is no Assertion Roulette type test smell as we ensure that in a test function, there should be only one \texttt{assert} for an element from the test array. However, we calculate repetitive test cases for the first research question, which covers duplicate assert-type test smells. The detail of this calculation will be in the next section.

\subsection{Evaluation}

We calculate different metrics for the first two research questions. Statement and branch coverage has been calculated for both research questions. For the first research question, we calculate additional metrics \ie Test Correctness and Repetition. In the following section, we are going to give a brief introduction to these metrics.
\begin{itemize}
    \item \textbf{Line coverage} or \textbf{statement coverage} is a common metric to measure the performance of software tester. This metric calculates how many lines have been covered by the unit tests out of the total number of lines. It can be formulated as $Statement~Coverage= \frac{Number~of~statements~executed}{Total~number~of~statements} \times 100$. Hence, if there are 20 statements in a module and 15 statements are executed using the unit tests. The statement coverage of these unit tests will be 75\%.
    \item \textbf{Branch Coverage} is the most well-known and practiced metric in software testing. A branch can happen mainly because of \texttt{if} condition in the code, but it also includes \texttt{loop}, \texttt{switch} cases \etc~Because of the branch, the execution of the program follows different parts of the source code. A good set of unit tests should cover all the branches. It follows a similar formula as statement coverage,   $Branch~Coverage= \frac{Number~of~branch~visited}{Total~number~of~branch} \times 100$. If there are eight branches and the unit tests visit five of them, the branch coverage of these unit tests will be 62.5\%.
    \item \textbf{Test Correctness and Repetition} Finally, we calculate the number of test correctness and repetitive unit tests. Usually, in the software development life cycle, unit tests should be written after having the requirement and before writing the actual code \latif{citation needed}. However, in our case, especially for the first research question, we performed a controlled experiment where the correctness of the codes was already vetted by the creator of the HumanEval dataset \cite{chen2021codex }and the other peers who used this dataset\latif{citation needed}. Hence, if the unit test is functionally correct, it should not fail ideally for a sample in the HumanEval dataset. For this reason, we calculate the number of GitHub Copilot-generated unit tests that failed. We also calculate the number of repetitive unit tests as they do not increase the coverage but affect the cost of generating and checking them.
\end{itemize}


The statement, branch coverage, and test correctness are calculated using \texttt{pytest} and \texttt{Coverage.py} tools. We calculate the number of repetitive unit tests from the generated unit tests array described in the previous sections by comparing them with each other.

\texttt{pytest} is used to execute the unit tests created by the GitHub Copilot, and \texttt{Coverage.py} is used to measure coverage by the unit tests. In this section, we will give a brief introduction to these tools.
\begin{itemize}
    \item \texttt{pytest} \cite{pytest} is a well-known testing framework for Python. It was first introduced in late 2002. It can be used to create a variety of software tests, including functional, end-to-end, unit, and integration tests. Its features include fixtures, assert re-writing, and parameterized testing. We use version 6.2.5 and its unit-testing functionality to evaluate the generated unit tests by GitHub Copilot.
    \item Python projects can have their code coverage evaluated using the utility \texttt{Coverage.py} \cite{coverage}. It keeps track of the code segments executed in your program while monitoring it; then, it examines the source code to find segments that should have been performed but weren't. In our work, we use the 6.5.0 version of this tool with \texttt{pytest} to calculate line and branch coverage.
\end{itemize}


For the last research question, we calculate the weighted average, $W$, of the unit tests with test smells for each test smell and project using this formula: 
\begin{equation}
    W = \frac{\sum_{n=1}^{\#~of~modules} \%~of~Tests~with~Smell}{ \sum_{i=1}^{\#~of~modules} Y_i}
\end{equation}

In this formula, we accumulate the percentage of unit tests with test smells and then divided by the sum of $Y_i$ where $Y_i$ is a function returns one if any of the unit tests in the module is containing the particular test smell and zero if the module is not containing the particular test smell. The formula for $Y_i$ is,\\
\[ Y_i =
 \begin{cases}
                                   0, & Module~not~Containing~Smell \\
                                   1, & Module~Containing~Smell 
  \end{cases}
\]



==> Files/ICPC/result_icpc.tex <==
\section{Results}\label{sec:result}

This section presents the results for each of our three research questions.


\input{Tables/RQ1.tex}

\subsection{RQ1: Code Elements}



\tblref{tab:result_rq1} presents the results for Python and Java. It reports the average \textit{line coverage} and \textit{branch coverage} for the unit tests generated by \pilot{} and the total number of correctly generated unit tests and repeated tests. These metrics are computed for each scenario (scenario 1 includes only  the function's code, scenario 2 includes the function's code and description, whereas scenario 3 includes code, description, and sample input-output).


% \subsubsection{Line and Branch Coverage}
As we can observe from this table,   the average line coverage \textit{increases} as we include more details in the function under test (used as context for test code generation). In the case of Java, however, the average line coverage was \textit{similar} across scenarios. 
In the case of branch coverage of the generated Python unit tests, we observe that this metric does not increase as more details are provided to GitHub Copilot -- the average branch coverage remained close to 30\% across the three scenarios. For Java Unit tests, we found that including sample input/outputs improved the branch coverage of the generated Unit tests by 14.5\%. 

% \subsubsection{Correct and Repeated Tests}
Moreover, we also found that out of 1,640 generated Python unit tests, the number of functional unit tests is \textit{increasing} for the presence of the description and sample input-output. However, the inclusion of the sample input-output also made GitHub Copilot generate more duplicate unit tests. From the table, we can see that in the third scenario, which includes the sample input-output in the code comment, at least 25\% samples out of 164 samples from the HumanEval dataset has duplicate unit tests in the 10 automated unit tests for each sample generated by GitHub Copilot. This observation is also similar to Java. We found that when we include sample input-output pairs (Scenario 3), the percentage of duplicate test cases is doubled compared to scenario 2. As shown in \tblref{tab:result_rq1}, 59 out of 160 samples had duplicate test cases in scenario 3.

We used GitHub Copilot to generate unit test functions for \texttt{pytest} and \texttt{JUnit}. We repaired the wrongly generated test functions.  For Python, we have to fix the issue for 4 samples out of 164 Python samples and 3 samples out of 160 Java samples. The common issue for the Python sample is that \pilot{} is not generating any code with the prompt; hence we have to write the test functions manually. For Java, instead of calling the targeted method to test, there is a calling for an unknown method; hence, we have to edit the targeted method name.

\begin{resultbox}
\textbf{\textbf{RQ1 Findings:}} 
\begin{itemize}[leftmargin=*]
    \item[--]  For Python, the inclusion of functional description and sample input-output pairs in the docstring can increase the line coverage for the unit tests generated by GitHub Copilot.  However, these code elements have no significant effect on branch coverage. For Java, the inclusion of both functional description and sample input-output pairs in the docstring can significantly increase the branch coverage, though it does not have any impact on line coverage.
    \item[--] The inclusion of functional descriptions and sample input-output improves the correctness of the generated test cases but, simultaneously, can lead to more duplicate unit tests for both programming languages.
\end{itemize}
\end{resultbox}


\subsection{RQ2: Comparison with Pynguin}
For this research question, we generated unit tests for 37 modules from 14 projects. We presented the result in Table \ref{tab:rq2}. For each project, we presented the average line and branch coverage.
% \joanna{confusing sentence for each coverage, we present the coverage?}. 
We also presented the weighted branch coverage for the modules we checked for 14 projects using Pynguin \cite{pynguinjournal} with Dynamic Many-Objective Sorting Algorithm (DynaMOSA) \cite{dynamosa} and without \textit{Type Hints}. According to Lukasczyk \etal \cite{pynguinjournal}, the DynaMOSA \cite{dynamosa} algorithm is the best performing algorithm for generating test cases. We use Pynguin without \textit{Type Hints}  as in our work GitHub Copilot has no explicit information about type for Python objects. Also, we presented results for 14 projects as Pynguin \cite{pynguinjournal}, they worked on \textit{python-semantic-release} project, but their tool has no result for this project. Besides, they only calculated branch coverage, not line coverage.


In total, we provided the average line and branch coverage per project. We found that the average line coverage ranged from 16.5\% to 100.0\%, and on average, it was 66.20\% per project. The branch coverage ranged from 7.25\% to 42.0\%, and on average, it was 25.35\% per project. Out of 162 unit tests for 37 modules, 48.65\% of them passed. Compared to the Pynguin \cite{pynguinjournal} result, there is no case where the coverage of unit tests generated by GitHub Copilot exceeds the performance of the branch coverage of using Pynguin \cite{pynguinjournal}. The average branch coverage by Pynguin \cite{pynguinjournal} is three times higher than the coverage with GitHub Copilot-generated unit tests. 

\begin{table*}[ht!]
\centering\footnotesize
\caption{Unit Tests Generated for Open-source Projects by GitHub Copilot}
\label{tab:rq2}
% \resizebox{1.85\columnwidth}{!}{%

\begin{tabular}{@{}|l| c|c|c|c|c|c|c|}\hline
\textbf{Project Name} & \textbf{\textbf{\#  Modules}} & \textbf{\# Test Cases} & \textbf{\# Passed} & \textbf{Line Coverage} & \textbf{Branch Coverage} & \textbf{Branch Coverage (Pynguin)} \\\hline
apimd (v1.2.1)&  1& 28 & 3(10.71\%) & 44.0\% & 15.0\%& 62.0\%\\
codetiming (v1.3.0) &1 & 2 &2(100\%) & 92.0\% & 38.0\%& 100.0\%\\
flake8 (v3.9.0) & 3 & 21&11(52.38\%) & 79.0\% & 35.33\%& 68.0\% \\
flutes (v0.3.0)&  1&1&1(100\%)&100.0\% & 30.0\% & 100.0\%\\
flutils (v0.7)& 3 & 17 &6(35.29\%) & 71.0\% & 13.33\%& 56.6\%\\
httpie (v2.4.0)&  4 & 4 &1(25\%) & 48.75\%&28.5\%& 73.0\%\\
isort (v5.8.0)&  2 &3 & 0(0\%) & 86.0\%& 32.0\%& 71.4\%\\
pdir2 (v0.3.2)&  4 &13& 5(38.46\%)&76.25\%&7.25\%& 68.0\%\\
py-backwards (0.7)& 4&9&5(55.56\%) &58.0\% &24.25\% & 42.7\%\\
python-string-utils (v1.0.0)&  2&38& 31(81.58\%)&44.0\%&16.0\%& 89.9\%\\
pytutils (0.4.1)& 5 &8& 4(50\%)&75.6\%&24.6\%& 84.4\%\\
sty (v1.0.0rc1)&  1&5&5(100\%)&100.0\%&42.0\%& 100.0\%\\
thonny (v3.3.6)&  4&9&4(44.44\%)&53.5\%&34.5\%& 54.5\%\\
typesystem (v0.2.4)&  2&4&1(25\%)&16.5\%&15.5\%& 53.0\%\\\hline
Total &  37&162&79(48.76\%)&65.22\%&24.38\%& 73.1\%\\\hline
\end{tabular}
 % }
\end{table*}

\begin{resultbox}
\textbf{\textbf{RQ2 Findings:}} 
\begin{itemize}[leftmargin=*]
\item[--] The average line coverage per project is 65.22\%, and the branch coverage is 24.38\% for the unit tests generated by GitHub Copilot for open-source Python projects. 
\item[--] About half of the unit tests passed (48.65\%) from the automatically generated unit tests by GitHub Copilot. 
\item[--] Pynguin \cite{pynguinjournal},  a state-of-the-art tool for the automated unit test generation tool for Python, has three times more average coverage than the branch coverage using unit tests generated by GitHub Copilot.

\end{itemize}
\end{resultbox}
\subsection{RQ3: Test Smells}
We checked \textbf{nine} test smells in 162 unit tests for the 37 modules from 14 projects.  Table \ref{tab:rq3} presents the weighted average for each test smell type and project in the table. The total row indicates the average for each project of a test smell, and in the bracket, we presented the total number of projects where the particular test smell is present.

From this table we can observe that Assertion Roulette (AR) is the most common test smell type in the generated unit tests by GitHub Copilot, and the second most common one is Magic Number Test (MNT). We did not find any Unknown Test (UT) in the generated unit tests by GitHub Copilot.

\textbf{Comparison to another study:} The distribution of the dataset for the empirical evaluation for Pytest-smell \cite{pytest_smell} followed this: Assertion Roulette, Magic Number Test, Conditional Logic Test, Duplicate Assert, Unknown Test, Exception Handling, Eager Test, Sleepy Test, and Redundant Print. Our finding matches the first two, and except for the Unknown Test, their top five and our top five are exactly the same but in a slightly different order. 

\begin{table*}[ht!]
\centering\footnotesize
\caption{Result for the Presence of Test Smells in the Generated Unit Tests by GitHub}
\label{tab:rq3}
% \resizebox{1.75\columnwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Project} & \textbf{AR} & \textbf{CLT} & \textbf{DA} & \textbf{EA}& \textbf{EH} & \textbf{MNT} & \textbf{RP} & \textbf{ST} & \textbf{UT} \\ \hline
apimd                  & 100.0\%  &  X & 100.0\% &  X & X  &  X  &  X & X  &  X \\ \hline
codetiming             &  X  & 50.0\% &  X&  X  & 50.0\%  & 100.0\% & X  & 100.0\% &  X \\ \hline
flake8                 &  X  & 57.14\% & X  &  X & 57.14\%& 7.14\%&   X& X  &   X\\ \hline
flutes                 & 100\%  &  X &  X&  X  & X  & 100\% & X  & X  &  X \\ \hline
flutils                & 65.08\%  & 71.43\% & 16.67\%&  X  & 71.43\%& 50.0\%  &  X &  X &  X \\ \hline
httpie                 & 100.0\%  & X  & 100.0\%&  X & X  & 100\% &  X &  X & X  \\ \hline
isort                  & 100.0\% &  X &  X &  X & X  & X   &  X &  X &  X \\ \hline
pdir2                  & 77.78\% &  X &  X &  X & X  & 33.33\%  & X  & X  & X  \\ \hline
py-backwards           & 91.75\%  &  X & X&  X   & X  & 33.33\%  & 66.67\%&  X & X  \\ \hline
python-string-utils    & 36.61\%  & X  & 12.5\%&  X &  X & 39.29\% &  X &  X & X  \\ \hline
pytutils               & 100.0\%  &  X & X &  X  &  X & 100.0\% & X  & X  &  X \\ \hline
sty                    & 100.0\%  & X  & X&  X   &  X & 100.0\% & X  &  X &  X \\ \hline
thonny                 & 100.0\%  & X  & X &  X  &  X & 66.67\% &  X &  X &  X \\ \hline
typesystem             & 100.0\%  & X  &  X &  X &  X & 83.50\% &  X &  X &  X \\ \hline
Total                  & 83.65\%(12) & 12.76\%(3) & 16.37\%(4)& 0.0\%(0)  & 12.78\%(3) & 57.99\%(12) & 4.76\%(1) &7.13\%(1) & 0.0\%(0) \\ \hline
\end{tabular}
% }
\end{table*}

\begin{resultbox}
\textbf{\textbf{RQ3 Findings:}}  
\begin{itemize}[leftmargin=*]
\item[--] Assertion Roulette and Magic Number Test are the most prevalent test smell found in the unit tests generated by GitHub Copilot. 
\item[--] There are also Conditional Logic Tests, Duplicate Assert, and Exception Handling test smells in these unit tests for open-source projects.
\end{itemize}
\end{resultbox}

==> Files/intro_old.tex <==
\section{Introduction}\label{sec:intro}


Automated code generation techniques based on Large Language Models (LLMs) generate code from  \textit{prompts}~\cite{allamanis2018survey}. These prompts specify the developer's intent and have varying level of granularity and structure. They may include sentences, code comments, code elements (\eg function signatures, expressions, \etc), or a combination of these. Thus, developers can write an initial code and/or comment and use these tools to generate the remaining code to speed up the software development process~\cite{albert22}. 
With the recent release of GitHub Copilot and ChatGPT, these techniques are increasingly being adopted in both industry and academic settings~\cite{albert22}.
% GitHub Copilot relies on a transformer-based \cite{attention2017} Large Language Model (LLM) fine-tuned for code generation.

With the increasing popularity of code generation LLMs, prior works investigated the correctness of the generated code~\cite{dakhel2022github}, their quality~\cite{siddiq2022empirical}, security~\cite{pearce2022asleep} and whether they can be used for API learning tasks \cite{apiicpc22}, and code complexity prediction \cite{siddiq23zero}. However, it is currently unclear the effectiveness of using prompt-based pre-trained code generation models to generate \textit{unit tests}. 

Unit testing  is an important software maintenance activity because it helps developers identify and fix  defects early; before they can propagate and cause more significant problems~\cite{rafi2012benefits,unittestsurvey,sina18unittest}. Moreover, unit tests help developers understand how the various code units in a software system fit together and work as a cohesive whole~\cite{moonen2008interplay}. Given its importance,  prior works  developed automated test case generation techniques~\cite{evosuite,ANAND20131978}.


To better understand the current capabilities of LLMs in generating unit tests, we conducted an empirical study using three LLMs (Codex~\cite{chen2021codex},  GPT-3.5-Turbo~\cite{chatgpt} and StarCoder \cite{li2023starcoder}) to generate JUnit5 tests for  classes in the HumanEval dataset's Java version~\cite{2023multilingual} and \nEvosuiteProjs{} open-source projects from the SF110 dataset~\cite{evosuite}. In this empirical study, we answered two research questions. In the first question, we used the full class under test as a context for the LLMs to generate unit test cases. In the second research question, we examine how different context styles (\eg only using the method under test, the presence, and absence of JavaDoc \etc) can influence the generated tests. We examined the produced tests with respect to their compilation rates, correctness, code coverage, and test smells. To the best of our knowledge, concurrent works (CODAMOSA \cite{lemieux@2023} and TestPilot \cite{schafer@2023}) are focused on the usefulness of LLM as a helper for search-based techniques and on weakly typed languages like Python and Javascript. Unlike these prior works,  our work investigates whether LLMs can be used off-the-shelf to generated unit tests for a strongly-typed language like Java> Moreover, we examine these generated tests in terms of their correctness, quality, as well as the effectiveness of different context styles when generating tests.


The \textbf{contributions} of our work are:
\begin{itemize}[leftmargin=*, noitemsep,topsep=0pt]
% \item A systematic study about proving context in the prompt inspired by Test-Driven Development approach to the LLM to generate unit tests.
\item A systematic study of three LLMs for zero-shot unit test generation for \nEvosuiteCUTs{} classes from \nEvosuiteProjs{} open-source projects in the SF110 dataset~\cite{SF100} and \nJavaHumanEval{} classes from the HumanEval dataset~\cite{2023multilingual}. 
\item An investigation of the quality of the produced unit tests by studying the prevalence of test smells in the generated unit tests by different code generation models.
\item A comparison of how different context styles affect the performance of LLMs in generating tests.
\item A  discussion about the implication of using code generation models for unit test generation in a Test Driven Development (TDD) environment.
\item A replication package with all the scripts used to gather the data and spreadsheets compiling all the results\footnote{\url{https://doi.org/10.5281/zenodo.10530787}}.
\end{itemize}



==> Files/relatedwork_old.tex <==
\section{Related Work}
\label{sec:related}
Prior research has concentrated on creating source code that can do a specific task automatically (code generation).
The deductive synthesis approach \cite{green69, manna2017}, in which the task specification is transformed into constraints, and the program is extracted after demonstrating the satisfaction of the constraints, is one of the foundations of program synthesis \cite{gulwani2017program}. Recurrent networks were used by Yin \etal \cite{yin2017} to map text to abstract syntax trees, which were subsequently coded using attention. Using the provided context, large language learning models have done a great job of producing source code. A variety of big language learning models have been made public to generate code (e.g., CodeBert \cite{codebert}, Codex \cite{chen2021codex}, and CodeT5 \cite{codet5}) after being refined on enormous code datasets. Later, GitHub Copilot developed an improved auto-complete mechanism using the upgraded version of Codex, which can help to solve fundamental algorithmic problems \cite{dakhel2022github}. Recent works~\cite{Aman22, codet,coderl2022} focuses on optimizing the process to create, fine-tune, and infer the Large Language Models-based code generation techniques. Using large language models for software test generation is not that common. Though they can be used for downstream tasks, for example, flaky test prediction \cite{fatima2022flakify}. However, recent work uses GPT-3 \cite{brown20} for software graphical interface testing \cite{guitesting23}. Our work is not focused on code generation but on how a publicly available code generation tool can be used for specialized tasks like unit test generation without fine-tuning.

Garousi and Mäntylä \cite{GAROUSI2016195} conducted a graduate-level study in software testing and pinpointed the most often used testing stages and methods. A total of 166 papers from the business and academic worlds are analyzed by Garousi and Küçük \cite{Vahid19}. The study's authors include information about prevention, detection, and correction and a list of test smells. The authors also offer a list of test smell-detecting instruments as part of their investigation. Pecorelli \etal \cite{pecorelli2022software} conducted an empirical study on software testing for android applications about finding effectiveness, design, and finding bugs in the production code. Wajdi \etal \cite{wajdi21} surveyed literature to fund the related testing tools and their detected smell. Fernandes \etal \cite{daniel21} made a comprehensive list of 20 test smells focusing on Python and announced four new test smell types.
In contrast, Weng \etal \cite{pynose} created a Python test smell detection and identified 17 diverse test smells. Pontillo \etal worked on detecting test smell using a machine learning model \cite{mltest}. Our work focused on the existing test smells' distribution in the generated unit tests by GitHub Copilot.


% ICSE 2022:
% GPT-3 for text generation
% Codex 

\joanna{Vinicius, add here}

There are several related works in the field of test generation. Some papers focused their research on unit test generation, such as~\cite{shamshiri@2015},~\cite{tufano@2020}, \cite{pacheco@2007}. Even though they have the same goal, those papers use different approaches. Paper~\cite{shamshiri@2015} proposes a search-based approach that automatically generates tests that can reveal functionality changes, given two program versions. On the other hand, paper~\cite{tufano@2020} proposes an approach that aims to generate unit test cases by learning from real-world focal methods and developer-written test cases. Finally, paper~\cite{pacheco@2007} present a technique that improves random test generation by incorporating feedback obtained from executing test inputs as they are created for generating unit tests.

Regarding papers with similar approaches, we found some papers that have based their solutions on Large Language Models (LLMs). There are three papers, such as~\cite{nashidretrieval@2023},~\cite{lemieux@2023},~\cite{schafer@2023}. Paper \cite{schafer@2023} uses Codex, an off-the-shelf LLM, to automatically generate unit tests for a given program without requiring additional training. On the other hand, work~\cite{lemieux@2023} combines the Search-based software testing (SBST) technique with the LLM approach. It explores whether Large Language Models (LLMs) of code, such as OpenAI’s Codex, can be used to help SBST's exploration. Finally, paper~\cite{nashidretrieval@2023} aims to devise an effective prompt that could help large language models with different code-related tasks.

Some papers have yet to propose something new regarding test generation in the literature but perform studies relevant to the area. For example, paper~\cite{bareiss@2022} performs a systematic study to evaluate how a pre-trained language model of code, CodeX, works with code mutation, test oracle generation from natural language documentation, and 
test case generation.

Finally, some papers propose different solutions for different problems in the area. Regarding test completion and looking for solutions to decrease time-consuming writing tests, paper \cite{nie@2023} proposes a deep learning model using code semantics for test completion. The work uses code semantics data, including the execution result of prior statements and the execution context of the test method. Regarding scalability and ensuring that all the code changes introduced into a code base are also tested, paper~\cite{qi@2010} proposes an
automatic test generation solution to this problem. It uses dynamic symbolic execution to generate a test input, which stresses the change.

Thus, the test generation field is a complex and broad study area. It has different approaches for different problems developed through the years, with relevant papers at least from 2007 with paper~\cite{pacheco@2007}. Our work is part of that diversity that also proposes a new approach, looking to evolve and contribute to the state-of-art of this study area.



\joanna{Ridwanul, add here}

Roy \etal presents DeepTC-Enhancer, a tool that uses Deep Learning and template-based methods to improve the readability of automatically generated test cases. The tool is evaluated with 36 developers, demonstrating its effectiveness in generating meaningful identifier names and documentation \cite{roy2020deeptc}.


Scalabrino \etal introduces BOT, an approach to adaptively allocate the search budget to classes in test case generation, and BRANCHOS, a method to predict branch coverage in a budget-aware way. The experiments show that BOT and BRANCHOS can significantly increase test coverage and effectiveness \cite{scalabrino2021adaptive}. 



Lin \etal examines the quality of identifiers in test code and finds that they are generally lower quality than in production code. The study also evaluates the limitations of current rename refactoring recommenders in improving test code identifiers \cite{lin2019quality}.


Soares \etal investigates open-source developers' awareness of test smells and their refactoring strategies. The study was conducted through a survey with 73 experienced open-source developers and the submission of 50 pull requests. The results show that developers acknowledge the negative impact of test smells and prefer most of the literature's proposals for their removal \cite{soares2020refactoring}.

Lemos \etal highlights the importance of software testing (ST) education in improving programming skills and code reliability. The study includes an experiment with senior-level computer science students and a survey of professors teaching introductory programming courses. The results indicate that software testing knowledge can improve code correctness by up to 20\%, but many instructors lack this knowledge \cite{lemos2018impact}. 


Leandro \etal introduces a technique for evaluating refactoring detection tools that involves applying a refactoring using an IDE and then checking if the tool can detect it. RefactoringMiner and RefDiff detected more refactorings in a percentage of the transformations, and the study revealed the need for a shared understanding of refactoring mechanics \cite{leandro2022technique}.


Vidaurre \etal discusses using genetic algorithms for generating unit tests and proposes a visual technique, TestEvoViz, to help practitioners analyze, compare, and tune the test generation process. The study shows that TestEvoViz is effective in improving the efficiency and effectiveness of unit testing \cite{cota2022testevoviz}.

    
Bergel \etal proposes a technique called Beacon that utilizes a Genetic Algorithm to automatically reproduce crashes in Python, which is challenging due to the lack of explicit type declarations in dynamic languages. The approach uses only the information contained in the error's stack-trace to generate the sequence of instructions needed to reproduce the crash. The study evaluates the proposed approach with three experiments, achieving a high precision while reproducing the desired crashes, and showing its independence of the language typing \cite{bergel2021beacon}. 



Bergel \etal presents Hapao, a test coverage tool implemented in Pharo Smalltalk, which uses visual representations and metrics to help programmers identify areas that require more testing. The results show that Hapao is effective in identifying gaps in test coverage and can assist in improving the quality of unit tests \cite{bergel2014increasing}.




Kashiwa \etal presents a large scale study with both quantitative and qualitative analysis to understand how different refactoring operations impact a system's test suites. The majority of refactoring operations do not induce test breaks, but some specific types such as "RENAME ATTRIBUTE" and "RENAME CLASS" have a higher chance of breaking test suites. Refactoring operations such as "ADD PARAMETER" and "CHANGE RETURN TYPE" often require additional changes to fix the test suite they break, even with modern IDEs that provide automated features \cite{kashiwa2021does}.


Pecorelli \etal presents  proposes a two-step systematic approach to generating unit tests: first creating tests that cover individual methods and then enabling the creation of intra-class tests targeting interactions among production code methods. Previous approaches using random or search-based algorithms did not ensure tests followed good design principles \cite{pecorelli2022toward}.



Pecorelli \etal presents a case study on the relationship between test-related factors and code quality in Apache systems. The study investigates how tests and different test-related factors relate to post-release defects. The key finding suggests that, when controlling for other metrics, test-related factors have limited connection to post-release defects \cite{pecorelli2021relation}.

Lambiase \etal highlights the negative impact of test smells on test maintainability and effectiveness. It proposes DARTS as a solution to detect and refactor three types of test smells using Intellij's APIs. By providing automated refactoring, DARTS can potentially save developers time and effort in maintaining their test suites \cite{lambiase2020just}.


Grano \etal examines the quality of test code generated by automated unit test generation tools. Seven test smells are used to measure code quality, and the diffuseness of these smells is evaluated in the test classes generated by three state-of-the-art tools. The study finds that these tools tend to generate a high quantity of two specific test smells that can negatively impact the reliability of production code \cite{grano2019scented}.



Camilli \etal introduces a testing framework that uses Markov Decision Processes to target uncertain components in software systems. The tester specifies uncertainty by attaching beliefs to transition probabilities, and Bayesian inference is used to update these beliefs based on testing evidence. The framework outperforms existing testing methods in terms of accuracy of the inference process \cite{9438600}.



Peruma \etal introduces tsDetect, an automated tool for detecting test smells in Java software systems. It discusses the architecture of the tool and its flexibility in incorporating new smell types and customizing existing detection rules. The paper also presents evaluation results showing high detection accuracy for tsDetect on a benchmark of 65 unit test files \cite{peruma2020tsdetect}. 


Li \etal discusses TeStereo, an automated tagging approach for methods in unit tests based on a catalog of stereotypes. The tagging is done through static control-flow, data-flow, and API call based analyses. The approach was evaluated through a study with students and a survey with Apache developers to validate the accuracy of the inferred stereotypes and measure their usefulness \cite{li2018aiding}.

Qusef \etal presents empirical evidence of the relation between the evolution of test smells and faults in the production code, based on a case study of Apache Ant. The study found that the absolute number of test smells increases as Apache Ant evolves and some test smells are positively correlated with the existence of faults in the production code. The study also showed that it is possible to predict faults in the production code based on the existence of test smells in the unit tests \cite{qusef2019exploratory}. 


Watson \etal presents a new approach called Atlas to automatically generate meaningful assert statements for test methods using Neural Machine Translation (NMT) based technique. Atlas was applied to thousands of test methods from GitHub projects and it was able to predict the exact assert statement manually written by developers in 31\% of the cases for top1 predicted assert, and 50\% for top-5 predicted assert statements. The approach has potential usefulness as a complement to automatic test case generation techniques and as a code completion support for developers \cite{watson2020learning}.



\textbf{\textcolor{red}{Noshin}}
\newline
Sebastiano Panichella \etal discusses the results of two different software testing competitions: the Java Unit Testing Competition and the Cyber-Physical Systems Testing Tool Competition. The competitions involved multiple tools and benchmarks, and the results were evaluated based on various metrics \cite{Zampetti_SBST2021}.

Florian Tambon \etal proposes a Probabilistic Mutation Testing (PMT) framework to address the verification and validation challenges of Deep Neural Networks (DNN). PMT leverages Bayesian estimation to define a probabilistic decision criterion to identify mutated models, and the evaluation shows that PMT can alleviate the flakiness issue of traditional DNN MT frameworks \cite{Foutse2023}.AmbieGen is a search-based test case generation framework for autonomous systems that identifies the most critical scenarios for a given system using evolutionary search proposed by Dmytro Humeniuk. It currently supports test case generation for autonomous robots and autonomous car lane keeping assist systems \cite{Foutse_AmbieGen2023}.

Fabiano Pecorelli \etal presents a study that investigates the effectiveness of manually written tests for Android apps. The study includes an analysis of the relation between test cases and defects in production code, a qualitative investigation with testing experts, and an exploration of design metrics for test cases. The results suggest that manually written tests have a low ability to detect defects in production code, and the study highlights the challenges faced by the research community in improving the effectiveness of testing \cite{Gemma2022}.

Chen Huo \etal proposes a new approach to interpret coverage information called direct and indirect coverage, which helps developers identify insufficiently tested code by focusing on methods that have a high proportion of indirectly covered entities. The paper also presents an empirical study of 17 real applications that demonstrates the effectiveness of the proposed approach and highlights the importance of considering inheritance and method overloading in testing \cite{Huo2016}.

Ding Li \etal proposes a technique extending prior techniques for test suit minimization that consumes up to 95\% less energy while maintaining coverage of the testing requirements \cite{Ding2014}. 

In their paper, YUE LIU \etal conducted an empirical study to evaluate the replicability, reliability, and explainability of automatic code generation models. They found that state-of-the-art approaches suffer from data duplication and input insensitivity, and that the models can recognize code grammar and structural information, but not key tokens that need to be updated. The study highlights the need for future work to improve the robustness and reliability of automated code generation models \cite{Liu2023}.

Mastropaolo \etal present an empirical study investigating whether semantically equivalent but different natural language descriptions result in the same recommended function when using GitHub Copilot to generate Java methods. Their results show that modifying the description results in different code recommendations in about 46\% of cases, and that differences in the descriptions might impact the correctness of the generated code. They highlight the importance of providing proper code descriptions to maximize the effectiveness of AI support in programming. Future work will focus on running controlled experiments with developers and improving automatic paraphrasing techniques for software-related text \cite{Mastropaolo2023}.

Davide Corradini \etal propose an automated black-box testing approach for detecting mass assignment vulnerabilities in RESTful APIs. Their approach uses clustering to identify read-only fields, and then generates concrete test cases to assess the execution of potential vulnerabilities. Their evaluation demonstrates a high accuracy in detecting seeded vulnerabilities across various programming languages, highlighting the importance of secure implementation in enforcing appropriate data access policies. Future work includes extending the approach to other types of programming defects and security vulnerabilities of REST APIs, as well as conducting user studies to improve reporting and fixing of defects \cite{Corradini2023}.

Emanuele Viglianisi \etal propose SOCRATES, an automated testing framework for smart contracts that deploys a society of bots to detect defects arising from multi-user interactions. The framework is able to expose both known and previously unknown faults in smart contracts that are actively run in the official Ethereum blockchain, and the use of multiple bots is more efficient in fault exposure than a single bot alone. The importance of accurate and thorough testing of smart contracts is highlighted, as they cannot be updated or patched once persistent in the blockchain. The reader is invited to refer to the original journal publication for a more complete presentation of SOCRATES \cite{Viglianisi2021}.

Dario Olianas \etal present STILE, a tool for parallel execution of Web test scripts that ensures compliance of execution schedules with dependencies among the involved test scripts, while minimizing the execution time and computation time. The experimental results show that STILE can halve the total execution time and the total CPU-time needed for full test suite execution. The paper also highlights the future work of estimating the optimal number of computation units required for a given test suite execution. The reader is invited to refer to the original journal publication for more details on STILE \cite{Olianas2021}.

Maurizio Leotta \etal investigated the impact of the Page Object (PO) design pattern on automated web testing. Their empirical study revealed that while POs do not compensate for the extra development effort in small test suites, they become more efficient with larger test suites (at least 10 times larger). The developers' skills also play a significant role in the benefits of PO adoption. The authors suggest future studies to measure the effects of the PO pattern during software and test suite evolution and conduct industrial case studies. 

Perplexity and burstiness are not applicable to this text as they are statistical language modeling metrics \cite{Leotta2020}.

Matthias Galster \etal presented their findings on the Second International Workshop on Variability and Complexity in Software Design. They discussed the challenges faced by software systems in accommodating various usage and deployment scenarios due to the increasing size and heterogeneity of software-intensive systems, critical operating conditions, and dynamic markets. The paper highlights the key themes for further investigation, including modeling variability, testing variability-intensive systems, and usability and scalability as cross-cutting concerns \cite{Matthias2022}.

In their paper, Jack van Heugten Breurkes and colleagues analyze the similarities between automated unit and acceptance testing practices in order to enable skill transfer across testing activities at different levels. They found that test-driven development (TDD) and model-based test generation (MBTG) are two practices widely researched for both unit and acceptance testing. While TDD encourages a design- and test-first mindset, which has a positive effect on the design of the system, MBTG requires additional manual effort to enable automated test generation. Future work includes running an online survey to validate the findings with practitioners \cite{Jack2017}.

Andrei Zlotchevski et al. propose exploring and evaluating transformer model fine-tuning for personalization in generating unit tests for Java methods. They consider three approaches: custom fine-tuning, lightweight fine-tuning, and prefix tuning, each offering a trade-off in total compute cost and predictive performance. Their empirical evaluation found that all customization strategies lead to significant model improvements on a target project, adapting to the coding style of the project, with each approach providing specific benefits in different deployment scenarios \cite{Andrei2022}.




%newline gulo bad deu sob , nahole error khabe , ami tanvir bad dichi


\textbf{\textcolor{red}{Fahmid}}
\newline
Mohammad Hamdaqa \etal present SmartHomeML, a domain-specific modeling language for smart home applications that allows users to define new skills independently from the target smart home provider. The language uses a rigorous metamodel and domain constraints to capture the syntax and semantics required to specify any smart home service, regardless of the platform or framework. SmartHomeML uses model-to-text transformation templates to generate smart home adaptation services that conform to the target provider specification, and supports automatic generation of a subset of smart home skills that conforms to Amazon Alexa and Samsung SmartThings APIs. The implementation of SmartHomeML and the sample application are available on Github.\cite{8039058}.

Mohammad Hamdaqa \etal proposed a classification scheme for vulnerabilities and code weaknesses in Ethereum smart contracts written in Solidity. By extracting 2143 vulnerabilities from various public coding platforms and vulnerability databases, they identified 11 categories for error source and 13 categories for potential impact. Their findings showed that language-specific coding and structural data flow are the dominant categories of vulnerabilities in Solidity smart contracts. They suggest that their classification scheme can support researchers in building tools and methods to avoid, detect, and fix smart contract vulnerabilities in the future. Future research should investigate generalization of the classification scheme to other blockchain networks and languages, explore more dimensions of the studied vulnerabilities and code weaknesses, and investigate ways in which the defined vulnerabilities and code weaknesses can be exploited. The authors acknowledge the support of the Icelandic Research Fund (Rann´ıs) grant number 207156-051. \cite{soud2022fly} 

Mohammad Hamdaqa \etal present iContractML 2.0, a second-generation smart contract language aimed at assisting developers in building smart contracts independently from the language or target blockchain platform. The language extends the first generation to support DAML and generates structural and deployment artifacts in addition to smart contract behavior. The paper demonstrates the capabilities of iContractML 2.0 through five case studies from different business domains. \cite{hamdaqa2022icontractml}


Neil Ernst \etal explore the hypothesis that architecture contributes to achieving continuous delivery and deployability goals. They summarize examples of deployability goals and architectural decisions made by three project teams practicing continuous delivery, and present deployability tactics collected from interviews in the form of an initial deployability tactic tree. The study emphasizes the importance of architectural design decisions to achieve deployability goals and suggests the need for clear understanding of stakeholder priorities and trade-offs. \cite{6903628}

%paper locked
Neil Ernst \etal propose that while Artificial Intelligence Driven Development Environments (AIDEs) hold immense potential in automating routine programming tasks, they also pose new challenges like bias, legal compliance, and security vulnerabilities that need to be addressed to ensure their effective use. Additionally, the impact of AIDEs on the learning of programming needs to be considered. \cite{9713901}

Neil Ernst \etal propose a model-driven framework that synthesizes aspect-oriented software development (AOSD) and model-driven engineering (MDE) to tackle software complexity and improve productivity. They use goal modeling to capture stakeholder concerns and AOSD language constructs to facilitate representation of multiple perceptions. The framework's applicability and usefulness were evaluated through a case study of an open-source e-commerce platform written in PHP, confirming their hypotheses. The authors suggest more in-depth studies and future research on the framework's automation support and handling functional aspects. This work can become a key enabler for more rigorous investigation in the area of AOSD and MDE synthesis\cite{storey2020software}

Nicolás Cardozo \etal propose LICCA, a tool for cross-language clone detection, which is integrated with the SSQSA platform. LICCA is evaluated on an extended set of cloning scenarios and is effective in clone detection for single languages, competing with state-of-the-art tools. LICCA is unique in cross-language clone detection, offering capabilities unavailable in existing tools. Future work includes improving precision, using alternative algorithms, and implementing filtering mechanisms to minimize false positives. LICCA is currently at the technology development level.\cite{8330250}

Nicolás Cardozo \etal present a run-time correctness verification approach for behavioral adaptations in software systems, using a symbolic execution engine to reason about reachable states of the system. The Kusasa engine generates an execution tree and identifies errors during the symbolic exploration of the tree, preventing erroneous states. The approach is a step towards ensuring run-time correctness, but further assessment and refinement are needed for more comprehensive case studies and improved performance. Assertions could also be explored to enhance correctness verification.
\cite{cardozo2014run}

Nicolás Cardozo and his team present a paper discussing the potential benefits and challenges of achieving a fully dynamic adaptive system using Context-oriented Programming (COP) and Reinforcement Learning (RL) techniques. The current COP techniques only allow for adaptations foreseen by developers at design time, while RL techniques lack modularity. Auto-COP, a recent proposal for automated adaptation generation, is presented as a starting point for achieving true run-time adaptation, with a roadmap and research agenda outlined for future work.\cite{cardozo2022next}

Nicolás Cardozo and his team present a paper discussing the potential benefits and challenges of achieving a fully dynamic adaptive system using Context-oriented Programming (COP) and Reinforcement Learning (RL) techniques. The current COP techniques only allow for adaptations foreseen by developers at design time, while RL techniques lack modularity. Auto-COP, a recent proposal for automated adaptation generation, is presented as a starting point for achieving true run-time adaptation, with a roadmap and research agenda outlined for future work\cite{ebert2021exploratory}


Nikolaos Tsantalis \etal propose an approach to automatically identify design and requirement self-admitted technical debt using Natural Language Processing (NLP). They analyzed the comments of ten open source projects and found that their approach significantly outperformed the current state-of-the-art based on fixed keywords and phrases. The study showed that words related to sloppy code or mediocre source code quality are the best indicators of design debt, whereas words related to the need to complete a partially implemented requirement in the future are the best indicators of requirement debt. They also found that their proposed approach can achieve a good accuracy even with a relatively small training dataset.\cite{da2017using}

Nikolaos Tsantalis \etal propose an approach to automatically identify Extract Method refactoring opportunities related to the complete computation of a given variable and the statements affecting the state of a given object. The approach includes rules to preserve existing dependencies and exclude refactoring opportunities that could possibly cause a change in program behavior. Evaluation results show that the proposed methodology successfully captures code fragments implementing a distinct functionality, resolves design flaws, improves method cohesion, and preserves program behavior. The proposed technique could also be applied to search-based refactoring approaches to find optimal \cite{tsantalis2011identification}

Nikolaos Tsantalis \etal propose a design pattern detection methodology based on similarity scoring between graph vertices. The approach can detect modified pattern versions, reduces the search space for large systems, and is extensible to novel patterns. Evaluation on three open-source projects demonstrates the accuracy and efficiency of the proposed method. The methodology automates the pattern detection process and fully extracts instances in a system for the patterns that the user is interested in, demonstrating high accuracy and precision.\cite{tsantalis2006design}

Oscar Chaparro \etal present Bee, an open-source tool integrated with GitHub that uses machine learning to automatically detect the type of user-written issues, identify and label sentences describing the system’s observed and expected behavior, and detect missing information in bug reports. Bee aims to improve bug report quality, assist developers on bug triage and resolution, and foster new research developments on automated bug management. The evaluation of Bee’s underlying models, using 5k+ bug reports, demonstrates its high accuracy in identifying the key elements in bug reports. (Perplexity and burstiness not used)\cite{song2020bee}

Oscar Chaparro \etal propose Euler, an approach for the automated quality assessment of steps to reproduce in bug reports, providing quality annotations and feedback to the reporters. Evaluators found Euler to be potentially useful in helping reporters improve their bug reports, with a high accuracy of identifying existing steps to reproduce, but with a moderate precision in identifying missing ones. Future improvements to Euler include improving the QRs and matching algorithm\cite{chaparro2019assessing}

The study by Oscar Chaparro \etal investigates the impact of different types of experimental radiation on the burrowing behavior and oxidative damage of the intertidal anemone A. hermaphroditica. The results indicate that UVB radiation causes these anemones to burrow faster and suffer higher levels of oxidative damage, while the presence of sediment provides protection against photo-oxidative damage. The study suggests that burrowing behavior is a key survival skill for these anemones, especially for juveniles. The authors recommend further research on the role of brooding in protecting embryos against UVB radiation. Perplexity and burstiness are not applicable in this context.\cite{cubillos2022effects}

The paper by Paris Avgeriou \etal proposes an approach to systematically and semiautomatically document architectural decisions, allowing for effective sharing among stakeholders. The Archium tool is presented as a first attempt to implement this approach, which weaves architectural decisions into architectural models and connects them to the implementation. The authors believe that treating architectural decisions with the same importance as architectural models will lead to significant progress in the field of software architecture. While empirical verification data is not yet available, ongoing industrial case studies are being conducted to validate the use cases and domain model, with plans to evolve Archium based on the outcome of these studies \cite{jansen2007tool}


Paris Avgeriou \etal conducted a systematic mapping study to explore documentation practices and challenges, as well as tooling used in Continuous Software Development (CSD). They found that poor documentation is a common issue in CSD due to informal communication, perception of documentation as waste, and short-term focus. They recommend using modern tools and technologies to improve documentation quality and applying the identified practices to mitigate challenges. The study also suggests further research on the combination and location of knowledge from multiple sources of truth in CSD. Finally, practitioners should consider using executable specifications and architecture frameworks tailored for CSD.\cite{theunissen2022mapping}

Paris Avgeriou \etal conducted the paradigm shift in software architecture from describing the outcome to documenting architectural knowledge has led to the need for managing architectural technical debt (ATD), which compromises system-wide quality attributes. However, ATD is often not effectively managed, leading to problems during maintenance and evolution. To address this, Paris Avgeriou et al. propose an ATD conceptual model and an architectural technical debt management (ATDM) process aligned with a general architecting process. Their contribution facilitates optimal decision making in architecture design and achieves a controllable and predictable balance between the value and cost of architecture design in the long term. Further research is needed in ATDM theory, ATDM tool support, and empirical evidence \cite{li2014architectural}

Paris Avgeriou and his team present PostFinder, an approach that helps programmers retrieve Stack Overflow posts relevant to their API function calls. By analyzing the project under development and optimizing the search process, PostFinder outperforms a well-established baseline and can be deployed to assist developers in selecting relevant Stack Overflow posts while they are programming. The approach also has potential to replace the module for searching posts in a code-to-code search engine \cite{rubei2020postfinder}

Rana Alkadhi and colleagues propose an approach for automatically extracting rationale from IRC messages of OSS communities. The study reveals that rationale is discussed in 25 percentage of IRC messages, with committers contributing to 54 percentage of the discussed rationale on average. Machine learning algorithms achieved 0.76 precision and 0.79 recall for binary classification, and an average of 0.45 precision and 0.43 recall for classification into finer-grained rationale elements\cite{alkadhi2018developers}

Rana Alkadhi et al. propose a method for improving the commit message writing process in software development by fine-tuning two transformer models for commit message generation and integrating them into popular code editors. Their method includes collecting and publishing a dataset of commit message and patch pairs for 6 programming languages, fine-tuning the generative language models, and providing integration with IntelliJ and VSCode. Their results show that their fine-tuned models perform significantly better than the base models for completion and generation tasks on a test dataset.\cite{miksik2023fine}

Robert Dyer \etal propose the creation of Software Engineer Collaboratories (SEClabs) to provide researchers with easily accessible and community-vetted research artifacts for evaluation purposes, thus enabling rapid advancement in software engineering research. SEClabs would function as a Collaboratory as a Service (CaaS) where research artifacts can be made publicly available and curated by the community. While there are challenges to its realization, the authors believe that SEClabs would provide researchers with a comprehensive and state-of-the-art experimental environment for empirical evaluations\cite{sherman2018software}

Mike Papadakis \etal present PIT, a practical and easy-to-use mutation testing tool for Java, that is well-integrated with development tools, open-source and actively maintained. PIT operates on bytecode, optimizes mutant executions and supports mutant operators conforming to current mutation testing research practices. In summary, PIT is a fast and scalable mutation testing tool that is applicable on real-world codebases, and publicly available \cite{coles2016pit}

Mike Robert Dyer \etal present a domain-specific language for mining source code at a large-scale, fine-grained level of detail, and with full history information. They demonstrate its usability by reproducing over 40 source code mining tasks from two large-scale previous studies with a reduction in code size and conducting a small controlled experiment on understanding the language features. This work provides a flexible data schema and supports all the features needed for mining source code, which can help answer research questions in fault prediction, change dependency, and temporal analysis on API and object usage. \cite{dyer2013declarative}

Mike Robert Dyer \etal present a domain-specific language for mining source code that supports large-scale, fine-grained level of detail and full history information, making it useful for research questions in fault prediction, change dependency, and temporal analysis on API and object usage. Their language is demonstrated to be effective by reproducing over 40 source code mining tasks from previous studies with a reduction in code size and conducting a small controlled experiment on language features. They propose a novel caching mechanism that incurs a relatively small overhead compared to existing approaches, and their intermediate language model and VM implementation give better support for dynamic AO features, showing the feasibility of supporting their IL model.\cite{setty2008weave}

The paper by Mike Rocco Oliveto \etal proposes incorporating test code quality metrics, such as test cohesion and coupling, as additional criteria for optimizing test case generation. Empirical studies demonstrate that this approach not only results in more cohesive and less coupled tests, but also increases branch coverage and results in statistically shorter tests. The authors define two textual-based test code metrics, CBTM and LCTM, and incorporate them into MOSA, a many-objective algorithm for automatic unit test generation. Future work includes evaluating the impact of this quality-based approach on the effectiveness of test cases and other maintainability factors. \cite{palomba2016automatic}


In their paper, Mike Rocco Oliveto \etal conducted a large-scale empirical study on automatically generated unit test classes and analyzed the diffusion of bad design solutions, called test smells. The study found that test smells are highly diffused in automatically generated unit test classes, with Assertion Roulette being the most frequent one. The study also found that test smells co-occur frequently and have strong positive correlations with structural characteristics of a system. The authors suggest that future research should focus on designing and developing new algorithms that balance branch coverage criteria with test code quality and automatically create text fixtures for test cases generated using existing tools.\cite{palomba2016diffusion}

The paper by Mike Rocco Oliveto \etal presents an empirical study that investigates the extent to which semantic-preserving changes in the natural language description provided to deep learning-based code generators have an effect on the generated code function. The study found that modifying the description results in different code recommendations in approximately 46 percent of cases, with differences in the semantically equivalent descriptions potentially impacting the correctness of the generated code by ±28percent. The results highlight the importance of providing a proper code description to maximize the effectiveness of AI support in programming. The authors suggest running a controlled experiment with developers to further investigate the impact of different code descriptions on the received recommendations.\cite{mastropaolo2023robustness}

The paper proposes BUGSJS, a benchmark of 453 real JavaScript bugs from 10 popular JavaScript server-side programs, accompanied by their bug reports, test cases, and patches. The lack of a common benchmark has limited the ability to fairly evaluate and compare the efficacy of new techniques in analyzing and testing JavaScript applications. BUGSJS provides a highly-reproducible platform for empirical studies and comparisons of JavaScript analysis and testing tools, and its flexibility allows for easy extensibility to other testing frameworks. Mike Rudolf Ferenc \etal. present this benchmark to facilitate future research in this area.\cite{gyimesi2019bugsjs}

In their paper, Mike Rudolf Ferenc \etal present FaultBuster, an automatic refactoring toolset that identifies problematic code parts via static code analysis, runs automatic algorithms to fix selected code smells, and executes integrated testing tools. FaultBuster was developed and tested in a 2-year project with 6 software development companies where thousands of code smells were identified and fixed in 5 systems having altogether over 5 million lines of code. By the end of the project, the companies refactored their systems with over 5 million lines of code in total and fixed over 11,000 coding issues, making FaultBuster a valuable tool for improving software quality through continuous refactoring. The authors plan to improve the tool in the future by extending it with more refactoring algorithms and improving the precision of the underlying issue checker.\cite{szHoke2015faultbuster}

Sebastiano Panichella \etal analyze the impact of build maintenance on developers by mining the version histories of 10 software projects. Their results show that build changes induce more relative churn on the build system than source code changes do on the source code. Furthermore, build maintenance yields up to a 27 percentage overhead on source code development and a 44percentage  overhead on test development. The authors suggest that project managers should account for build maintenance in their plans and budgets, and future studies should consider analyzing work items to accurately represent the unit of development work. They also plan to investigate the advantages and disadvantages of different build ownership styles\cite{mcintosh2011empirical}

Sebastiano Shane McIntosh and his colleagues conducted an analysis of the build maintenance overhead on developers by mining version histories of one proprietary and nine open source projects. Their results indicate that build maintenance imposes up to a 27percentage overhead on source code development and a 44percentageoverhead on test development. The build system churn rate is comparable to that of the source code, and build changes induce more relative churn on the build system than source code changes induce on the source code. Project managers should explicitly account for build maintenance in their project plans and budgets. The paper concludes by suggesting future coevolution studies consider analysis at the work item level and investigate the advantages and disadvantages of different build ownership styles.\cite{mcintosh2012evolution}

Shin Yoo \etal. have presented a comprehensive survey on test oracles, including specified, derived, and implicit oracles. They have analyzed publication trends and discussed two noteworthy and promising research directions: test oracle reuse and test oracle metrics. Oracle reuse is important and promising, with two approaches being generalizations of reliable reset and sharing of oracular data across software product lines. Test oracle metrics are a challenge and an opportunity for the software metrics community, allowing testers to assess the features offered by alternative test oracles.\cite{barr2014oracle}

Regression testing is a testing activity that is performed to provide confidence that changes do not harm the existing behaviour of the software. Test suites tend to grow in size as software evolves, often making it too costly to execute entire test suites. A number of different approaches have been studied to maximize the value of the accrued test suite: minimization, selection and prioritization. Test suite minimization seeks to eliminate redundant test cases in order to reduce the number of tests to run. Test case selection seeks to identify the test cases that are relevant to some set of recent changes. Test case prioritization seeks to order test cases in such a way that early fault detection is maximized. This paper surveys each area of minimization, selection and prioritization technique and discusses open problems and potential directions for future research.\cite{yoo2012regression}

In their paper, Shin Yoo \etal provide a thorough overview of techniques for oracle automation in software testing, including modelling, specifications, contract-driven development, and metamorphic testing. They also emphasize the importance of reducing cost and increasing benefit in all forms of oracle. The paper concludes with a roadmap for future work at the interfaces between existing definitions of oracles. The authors have also made a repository of papers on oracles available to the community.\cite{harman2013comprehensive}

Shinpei Hayashi \etal propose a theory of modeling by defining a canonical set of relations and a graphical syntax to represent them. The paper also introduces a test-driven development method for model-to-model transformations, focused on maintaining test relevance and improving maintainability through formal notations.\cite{moiseev2009generating}

Simone Scalabrino \etal present an empirical study investigating the robustness of GitHub Copilot, a deep learning-based code generator. The study shows that modifying natural language descriptions of code components results in different code recommendations in 46 percentage of cases, and some correct recommendations can only be obtained using specific descriptions. This highlights the importance of providing proper code descriptions to maximize the effectiveness of AI support in programming\cite{mastropaolo2023robustness}

Simone Scalabrino \etal explore the usage of the Text-To-Text Transfer Transformer (T5) architecture for code-related tasks. The T5 model is pre-trained on a large dataset and then fine-tuned on specialized datasets for tasks such as automatic bug fixing and code comments generation. The results show that the T5 model outperforms the four baselines for the four tasks. However, the authors suggest further investigations to better understand what makes T5 perform better, and note that the reported results are a lower bound of T5 capabilities. Code and data used in the study are publicly available.\cite{mastropaolo2021studying}

Simone Scalabrino and colleagues conducted a study comparing the readability of manually written and automatically generated test cases with the corresponding classes under test. Their results showed that developers tend to neglect the readability of test cases and that automatically generated test cases are generally less readable than manually written ones, opening new research directions to improve the quality of test cases.\cite{grano2018empirical}

Tracy Hall \etal conducted an exploratory study on the skill-based errors made by software developers and their mitigation strategies. They found that complex development environments and difficulties in maintaining focus were common reasons for errors, and developers relied mostly on improving their own willpower to mitigate them. The authors suggest that a Swiss Cheese approach may help prevent errors from causing serious failures in software development.\cite{nagaria2020software}

Tracy Hall \etal found that JUnit tests are not always effective in detecting defects in software systems, and suggest that more tests that touch related methods are needed. The study also identified method count and average lines of code as good predictors of JUnit test effectiveness. The authors recommend identifying more features of good unit tests to improve software quality. Further analysis on commercial systems and investigating relationships between defect types and unit test features are planned for future work.\cite{petric2018effectively}

In this study, Tse-Hsun (Peter) Chen \etal propose an unsupervised framework, StrucTexVec, which incorporates both textual and structural information to enhance pre-trained code embeddings for software engineering tasks. The authors evaluate seven code embedding techniques on six downstream tasks and find that pre-trained embeddings can generally improve performance, but different techniques can result in diverse results. The study highlights the importance of careful consideration when selecting embedding techniques for SE tasks and suggests opportunities for future research to improve these techniques.\cite{ding2022can}

Tse-Hsun (Peter) Chen \etal present T-Evos, a dataset on test result and coverage evolution in 12 open-source Java projects, covering 8,093 commits. They conduct an empirical study to analyze the characteristics of test failures in a CI setting and find that failures are frequent, with some taking weeks to resolve, highlighting the relationship between code changes and test failures, and providing insights for future automated testing research. The dataset is useful for future testing research and benchmarking in CI.\cite{chen2022t}

Vincenzo Riccio \etal propose a strategy to enhance the capability of test sets to detect faults in deep learning (DL) models. Their tool DeepMetis generates new test inputs that simulate real DL faults and increase the detection capability of the test set by 63 percentage on average. The approach is effective in exposing unseen mutants, indicating the occurrence of yet undetected faults\cite{riccio2021deepmetis}

In their paper, Vincenzo Riccio \etal propose juGULAR, a hybrid automated GUI exploration technique that combines automated exploration with Capture and Replay. By leveraging Machine Learning classifiers to detect Gate GUI instances and user-provided input event sequences to unlock them, juGULAR can improve app exploration while minimizing human intervention. The technique was validated through an experiment involving 14 real Android apps, demonstrating improved coverage and network traffic generation compared to the state-of-the-practice tool Monkey. Future work will address non-deterministic Gate GUIs and extend the technique to consider more Gate GUI classes. The authors also plan to extend the validity of their experimental results through an industrial case study.\cite{amalfitano2019combining}

This paper locked \cite{specificationinvited}

In this paper, Wahab Hamou-Lhadj \etal propose CLEVER (Combining Levels of Bug Prevention and Resolution Techniques), an approach that can detect risky commits with 79.10 percentage precision and 65.61 percentage recall. CLEVER uses code metrics, clone detection techniques, and project dependency analysis to detect risky commits within and across projects, and operates at commit-time. It not only detects risky commits but also recommends fixes to developers. The authors believe that CLEVER is a practical approach that can integrate well with the developer’s workflow. As future work, they plan to build a feedback loop between users and clusters of known buggy commits, improve CLEVER to deal with generated code, and investigate how to improve the proposed fixes.\cite{nayrolles2018clever}


Xin Xia \etal propose DeepCom, an approach to generate code comments for Java methods using natural language processing techniques and a deep neural network. DeepCom outperforms the state-of-the-art by a substantial margin, achieving better results on a machine translation metric. The authors plan to introduce more domain-specific customizations and apply DeepCom to other software engineering tasks in future work.\cite{hu2018deep}

The paper proposes a dual training framework that exploits the correlation between code summarization and code generation tasks to improve the performance of both. The framework considers dualities on probability and attention weights and applies corresponding regularization terms to constrain the duality. Experimental results demonstrate its effectiveness over baselines on two datasets from GitHub. Xin Xia \etal propose a dual training framework to improve the performance of code summarization and code generation tasks by exploiting their correlation in their paper\cite{wei2019code}

Xin Xia \etal propose Hybrid-DeepCom, a machine learning-based approach to generate code comments for Java methods. By combining lexical and structural information, Hybrid-DeepCom outperforms existing methods on machine translation and information retrieval metrics. The paper also addresses challenges such as code structure learning and reducing out-of-vocabulary tokens. In future work, the authors plan to customize the approach for other software engineering tasks.\cite{hu2020deep}

Alberto Martin-Lopez et al. compare black-box and white-box test case generation approaches for RESTful APIs using RESTest and EvoMaster tools, respectively. They also propose integrating both approaches by using black-box test cases as a seed for white-box search-based test case generation. Results show that there is no one-size-fits-all strategy, and the combination of both approaches yields the best results in most case studies. The paper provides lessons learned and open challenges for guiding the further development of current tool support.\cite{martin2021black}

Alberto Martin-Lopez et al. propose RESTest, a black-box testing framework for RESTful APIs that supports the automated analysis of inter-parameter dependencies. RESTest enables the use of constraint solvers for efficient generation of valid test cases, resulting in the detection of more faults and faster testing. Evaluation results show that RESTest can generate up to 99% more valid test cases than random testing and revealed 2K failures undetected by random testing, uncovering bugs in all services tested.\cite{martin2020restest}

Alberto Martin-Lopez et al. propose a domain-specific language called Inter-parameter Dependency Language (IDL) for the automated analysis of inter-parameter dependencies in web APIs. They present a mapping to translate an IDL document into a constraint satisfaction problem (CSP), enabling the automated analysis of IDL specifications. Their approach is supported by an editor, a parser, an OAS extension, an analysis library (IDLReasoner), and a test suite. The proposed tool suite has the potential to automate the management of inter-parameter dependencies in web APIs, opening new research opportunities in areas such as code generation and testing.\cite{martin2021specification}

Romain Robbes et al. evaluated the code synthesis capabilities of the Codex model on 115 Python problem statements from HackerRank. Their study shows that while Codex is proficient in Python, it exhibits clear signs of generating memorized code, which is alarming considering the potential impact on future code production. They propose a framework for code-synthesis evaluation using variations of problem statements based on mutations. The study also highlights issues with scientific evaluations and the potential risks associated with large-scale source code models.\cite{karmakar2022codex}

Romain Robbes et al. evaluated the Codex model's code synthesis capabilities based on 115 Python problem statements from HackerRank. They found that Codex solved 96 percentage  of the problems in a zero-shot setting and 100percentage  in a few-shot setting. However, the evaluation also showed that Codex generated memorized code, which is concerning because it could impact how code is produced in the future. They proposed a framework for code-synthesis evaluation using variations of problem statements based on mutations. In conclusion, additional investigation is necessary as the use and adoption of Codex and other large source code language models as foundation models can have a far-reaching impact on the way future code is produced, maintained, and used.Romain Robbes et al. proposed a benchmark to assess the quality of approaches to find traceability links between source code and emails. They devised and evaluated several lightweight methods to find traceability links, which showed that such approaches can achieve significant results in terms of accuracy. This indicates that heavyweight techniques may not be necessary to achieve good results in finding traceability links between source code and emails. The benchmark can also be used to train learning algorithms and test new approaches.\cite{bacchelli2009benchmarking}

Romain Robbes et al. explore the applicability of pre-trained transformer models in downstream software engineering tasks. They propose four probing tasks to identify deficiencies in code properties and analyze model layers' characteristics. Their study includes BERT, CodeBERT, CodeBERTa, and GraphCodeBERT and finds that while GraphCodeBERT is more consistent, BERT surprisingly performs well on some code tasks, indicating the need for further investigation. The study highlights the potential of transformer models in SE tasks and the importance of evaluating their effectiveness through diagnostic tasks.\cite{karmakar2021pre}



==> Tables/smells.tex <==
% \begin{table*}[ht!]
% \centering\scriptsize
% \caption{The Analyzed Test Smells in Java}
% \label{tab:test-smell}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \textbf{Acronym} & \textbf{Test Smell} & \textbf{Description} & \textbf{Source} \\ \hline
% AR & Assertion Roulette & Multiple unexplained assertions in the same test method & Deursen \etal \cite{Simula.SE.525} \\ \hline
% CI & Constructor Initialization & Test class with constructor method and field initialization & Peruma \etal \cite{peruma19}  \\ \hline
% CLT & Conditional Logic Test & Test methods that contain conditional statements & Meszaros \etal \cite{meszaros03} \\ \hline
% DA & Duplicate Assert & More than one of the same verification method that checks the same parameters & Peruma \etal \cite{peruma19}  \\ \hline
% % DE & Dependent Test & Call other test methods from the test method & Peruma \etal \cite{peruma19}  \\ \hline
% DT & Default Test & Automatically generated test class with default name & Peruma \etal \cite{peruma19}    \\ \hline
% EA & Eager Test & Test method that checks many methods of the object to be tested & Deursen \etal \cite{Simula.SE.525} \\ \hline
% EH & Exception Handling & When an exception handling is performed within a test method. & Peruma \etal \cite{peruma19}  \\ \hline
% EM & Empty Test & Test method without executable statements & Peruma \etal \cite{peruma19}   \\ \hline
% GF & General Fixture & Setup method fields that are not used in all test methods & Deursen \etal \cite{Simula.SE.525}     \\ \hline
% IT & Ignored Test & When a test method is ignored through the framework's annotation & Peruma \etal \cite{peruma19}     \\ \hline
% % LC & Lack of Cohesion of Test Cases & Test cases are grouped together in one test suite but are not cohesive & Greiler \etal \cite{greiler13}     \\ \hline
% LT & Lazy Test & Several test methods that verify the same production method & Deursen \etal \cite{Simula.SE.525}    \\ \hline
% MG & Mystery Guest & When a test method uses and depends on external resources & Deursen \etal \cite{Simula.SE.525}    \\ \hline
% MNT & Magic Number Test & Test Method that contains some number without indicating their purpose & Meszaros \etal \cite{meszaros03}  \\ \hline
% % NS & Non-Functional Statement & When there is an empty scope within a test method. & Fernandes \etal \cite{daniel21} \\ \hline
% % OIS & Obscure In-Line Setup & Test case contains too many setup steps & Greiler \etal \cite{greiler13}     \\ \hline
% % PPB & Programming Paradigms Blend & When there are fields initialized outside the test class (global scope) and used in the test class & Fernandes \etal \cite{daniel21} \\ \hline
% RA & Redundant Assertion & Test method with checks that always have the same response & Peruma \etal \cite{peruma19}      \\ \hline
% RO & Resource Optimism & Test method that optimistically assumes the state of an external resource as available & Deursen \etal \cite{Simula.SE.525}    \\ \hline
% RP & Redundant Print & Test method containing screen print statements & Peruma \etal \cite{peruma19}  \\ \hline
% SE & Sensitive Equality & Use toString method in a test method to make validations & Deursen \etal \cite{Simula.SE.525}    \\ \hline
% ST & Sleepy Test & Test method with pauses to wait for an event & Peruma \etal \cite{peruma19}   \\ \hline
% % TM & Test Maverick & Test suite has a fixture with setup, but a test case in this suite does not use this setup & Greiler \etal \cite{greiler13}     \\ \hline
% % UDT & Undefined Test & It occurs when the name of a test method is not prefixed with “test”. & Fernandes \etal \cite{daniel21}  \\ \hline
% UT & Unknown Test & Test method without assertion & Peruma \etal \cite{peruma19}  \\ \hline
% % VSM & Verifying in Setup Method & When there is an assertion method within the SetUp method. & Fernandes \etal \cite{daniel21} \\ \hline
% VT & Verbose Test & Test method with many lines of code & Meszaros \etal \cite{meszaros03}  \\ \hline
% \end{tabular}
% \end{table*}

\begin{table}[ht!]
\centering\scriptsize
\caption{Test Smells Detectable by \textsc{TsDetect}~\cite{peruma2020tsdetect}}
\label{tab:test-smell}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{@{}lp{5.6cm}@{}}
\toprule
\multicolumn{1}{c}{\textbf{\textbf{Test Smell}}} & \multicolumn{1}{c}{\textbf{\textbf{Description}}}                                                                                   \\ \midrule
Assertion Roulette (AR)                          & Multiple unexplained assertions in the same test method~\cite{Simula.SE.525}                                                        \\
Constructor Initialization (CI)                  & Test class with constructor method and field initialization~\cite{peruma19}                                                         \\
Conditional Logic Test (CLT)                     & Test methods that contain conditional statements~\cite{meszaros03}                                                                  \\
Duplicate Assert (DA)                            & More than one of the same verification method that checks the same parameters~\cite{peruma19}                                       \\
Default Test (DT)                                & Automatically generated test class with default name~\cite{peruma19}                                                                \\
Dependent Test (DPT)                                & Test being executed depends on other tests’ success\cite{peruma19}                                                              \\
Eager Test (EA)                                  & Test method that checks many methods of the object to be tested~\cite{Simula.SE.525}     \\
Exception Handling (EH)                          & When an exception handling is performed within a test method~\cite{peruma19}                                                        \\
Empty Test (EM)                                  & Test method without executable statements~\cite{peruma19}                                                                           \\
General Fixture (GF)                             & Setup method fields that are not used in all test methods~\cite{Simula.SE.525}           \\
Ignored Test (IT)                                & When a test method is ignored through the framework's annotation~\cite{peruma19}                                                    \\
Lazy Test (LT)                                   & Several test methods that verify the same production method~\cite{Simula.SE.525}         \\
Mystery Guest (MG)                               & When a test method uses and depends on external resources~\cite{Simula.SE.525}          \\
Magic Number Test (MNT)                          & Test Method that contains some number without indicating their purpose~\cite{meszaros03} \\
Redundant Assertion (RA)                         & Test method with checks that always have the same response~\cite{peruma19}                                                          \\
Resource Optimism (RO)                           & Test method that optimistically assumes the state of an external resource as available                                              \\
Redundant Print (RP)                             & Test method containing screen print statements~\cite{peruma19}                                                                      \\
Sensitive Equality (SE)                          & Use toString method in a test method to make validations~\cite{Simula.SE.525}            \\
Sleepy Test (ST)                                 & Test method with pauses to wait for an event~\cite{peruma19}                                                                        \\
Unknown Test (UT)                                & Test method without assertion~\cite{peruma19}                                                                                       \\
Verbose Test (VT)                                & Test method with many lines of code~\cite{meszaros03}                                    \\ \bottomrule
\end{tabular}
\end{table}
